Efficient Exploration through Bayesian Deep Q-Networks

We study reinforcement learning (RL) in high dimensional episodic Markov decision processes (MDP). We consider value-based RL when the optimal Q-value is a linear function of d-dimensional state-action feature representation. For instance, in deep-Q networks (DQN), the Q-value is a linear function of the feature representation layer (output layer). We propose two algorithms, one based on optimism, LINUCB, and another based on posterior sampling, LINPSRL. We guarantee frequentist and Bayesian regret upper bounds of O(d sqrt{T}) for these two algorithms, where T is the number of episodes. We extend these methods to deep RL and propose Bayesian deep Q-networks (BDQN), which uses an efficient Thompson sampling algorithm for high dimensional RL. We deploy the double DQN (DDQN) approach, and instead of learning the last layer of Q-network using linear regression, we use Bayesian linear regression, resulting in an approximated posterior over Q-function. This allows us to directly incorporate the uncertainty over the Q-function and deploy Thompson sampling on the learned posterior distribution resulting in efficient exploration/exploitation trade-off. We empirically study the behavior of BDQN on a wide range of Atari games. Since BDQN carries out more efficient exploration and exploitation, it is able to reach higher return substantially faster compared to DDQN.

==> Sections/3-Preliminaries.tex <==
\section{Preliminaries}
An infinite horizon $\gamma$-discounted MDP $M$ is a tuple $\langle \X, \A, T, R,\gamma\rangle$, with state space $\X$, action space $\A$, and the transition kernel $T$, accompanied with the reward function of $R$ where $0<\gamma\leq 1$. At each time step $t$, the environment is at a state $x_t$, current state, where the agent needs to make a decision $a_t$ under its policy. Given the current state and action, the environment stochastically proceed to a successor state $x_{t+1}$ under probability distribution $T(X_{t+1}|x_t,a_t):=\Prob(X_{t+1}|x_t,a_t)$ and provides a stochastic reward $r_t$ with mean of $\E[r|x = x_t,a= a_t] = R(x_t,a_t)$. In the following, $\|\cdot\|_2$ denotes the spectral norm and for any positive definite matrix $\chi$, $\|\cdot\|_{\chi}$ denotes the  $\chi$ matrix-weighted spectral norm. For any natural number $H$,  $[H]=\lbrace 1,2, \ldots,H\rbrace$. Since it is mainly clear from the context, to ease to notation, we mainly use the same notation for random variables and their realizations. 
In RL, the agent objective is to optimize the overall expected discounted reward over the policies $\pi:=\X \rightarrow \Delta_\A$, stochastic mappings from states to actions,  $\pi(a|x) := \Prob(a|x)$.
\begin{align*}%\label{eq:eta}
\eta^*\!=\!\eta(\pi^*) \!=\! \max_{\pi}\eta(\pi)\!= \!\max_{\pi}\lim_{N\rightarrow\infty}\E_{\pi}\left[\sum_{t=0}^N \gamma^tr_t\right]
\end{align*}
where the expectation is under the stationary distribution with respect to the randomness in the distribution of initial state, transition probabilities, stochastic rewards, and policy. The $\eta^*$ and $\pi^*$ are optimal expected return and optimal policy, respectively resulting in the optimal $Q$ function; 
%%We denote the the slotuionreturn under optimal policy $\pi^*$ as $\eta^*$.
%%Let $V_{\pi}(x)$ denote the average discounted reward under policy $\pi$ starting off from state $x$, and $Q_{\pi}(x,a)$ denote the same value starting form state $x$ but taking action $a$.
%%
%Let $Q_{\pi}(x,a)$ denote the average discounted reward under policy $\pi$ starting off from state $x$ and taking action $a$ in the first place.
%\begin{align*}
%Q_{\pi}(x,a) := \lim_{N\rightarrow\infty}\E_{\pi}\left[\sum_{t=0}^N \gamma^tr_t|x_0 = x,a_0=a\right]
%\end{align*}
% \begin{align*}
% &V_{\pi}(x) := \lim_{N\rightarrow\infty}\E_{\pi}\left[\sum_{t=0}^N \lambda^tr_t|x_0 = x\right]\\
% &Q_{\pi}(x,a) := \lim_{N\rightarrow\infty}\E_{\pi}\left[\sum_{t=0}^N \lambda^tr_t|x_0 = x,a_0=a\right]
% \end{align*}
%with the optimal policy and corresponding $Q$ function;
%For a given policy $\pi$ and Markovian assumption of the model, we rewrite the equation for the Q functions as follows:
%\begin{align}\label{eq:bellman}
%\!\!\!Q_{\pi}(x,a)\! = \!R(x,a) \!+\!\gamma \!\sum_{x',a'}\!\!\!T(x'|x,a)\pi(a'|x')Q_{\pi}(x',a')
%\end{align}
%To find the optimal policy, one can solve a linear programming problem in Eq.~\ref{eq:eta} or follow the corresponding Bellman equation Eq.~\ref{eq:bellman} where both of the optimization methods solve the following 
\begin{align*}
Q^*(x,a) = R(x,a) + \gamma\E_{x'}\left[\max_{a'}Q^*(x',a')|x,a.\right]
\end{align*}
%$\forall x,a$, $Q^*(x,a) = Q_{\pi^*}(x,a)$ and the optimal policy is a deterministic mapping from state to actions in $\mathcal{A}$, i.e. $x\rightarrow arg\max_{a}Q^*(x,a)$. 
%In RL, we do not know the transition kernel and the reward function in advance, therefore, we cannot solve the posed Bellman equation directly. 
In order to estimate the optimal $Q$ function, minimizing the Bellman residual 
\begin{align}
\L(Q) = \E_{\pi}\left[\left(Q(x,a)-r-\gamma Q(x',a')\right)^2\right]
\end{align}
has been proposed~\citep{schweitzer1985generalized,lagoudakis2003least,antos2008learning}.
where the tuple $(x,a,r,x')$ consists of consecutive samples under behavioral policy $\pi$. \citet{mnih2015human} carries this idea, and introduce Deep Q-Network (\DQN) where the Q-function is represented using a deep network. To improve the quality of $Q$ estimate, they use back propagation on loss $\L(Q)$ using the TD update \citep{sutton1998reinforcement} which results in a bias estimator of the $Q$ function. In the following we describe the setting used in \DDQN. In order to reduce the bias of the estimator, they introduce target network $Q^{target}$ and target value $y=r+\gamma Q^{target}(x',\hat{a})$ where $\hat{a} = \arg\max_{a'}Q(x',a')$ with a new loss $\L(Q,Q^{target})$
\begin{align}\label{eq:reg}
\L(Q,Q^{target}) = \E_{\pi}\left[\left(Q(x,a)-y\right)^2\right]
\end{align}
This regression problem minimizes the estimated loss $\wh\L(Q,Q^{target})$, which minimizes the distance between the $Q$ and the target $y$. A \DDQN agent,  once in a while updates the $Q^{target}$ network by setting it to $Q$ network, pursues the regression with the new target value and provides a biased estimation of the Q-value.

%In practice we are able to estimate the loss $\wh\L(Q,Q^{target})$ which tries find a Q-function which matches the target value. This loss function provides unbiased estimation of the gradient with respect to network parameter in order to minimize the loss.





==> Sections/3.1-TSvsE.tex <==
%\vspace*{-0.5cm}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\begin{table*}[t]
  \centering
  \caption{Characteristics of Thompson Sampling, $\varepsilon$-greedy, and Boltzmann exploration what information they use for exploration}
  \footnotesize
%   \hspace*{-1.cm}
  \begin{tabular}{l|c|c|c}
    % \multicolumn{1}{c}{}&\multicolumn{2}{c}{} \\
    \toprule
 Strategy  & Greedy-Action  & Estimated $Q$-values  &  Estimated uncertainties \\
  \midrule
$\varepsilon$-greedy &\cmark &\xmark&\xmark \\
\midrule
Boltzmann exploration &\cmark&\cmark&\xmark \\
\midrule
Thompson Sampling &\cmark&\cmark&\cmark \\
    \bottomrule
  \end{tabular}
  \label{table:reasons}
\end{table*}
% \vspace*{-0.5cm}



\section{Why Thompson Sampling and not \texorpdfstring{$\varepsilon$}{}-greedy or Boltzmann exploration}

In  value approximation RL algorithms,  there are different ways to manage the exploration-exploitation trade-off.  \DQN uses a naive $\varepsilon$-greedy for exploration, where with $\varepsilon$ probability it chooses a random action and with $1-\varepsilon$ probability it chooses the greedy action based on the estimated $Q$ function. Note that there are only point estimates of the $Q$ function in \DQN. In contrast, our proposed Bayesian approach \bdqn maintains uncertainties over the estimated $Q$ function, and employs it to carry out Thompson Sampling based exploration-exploitation. 
%
Here, we demonstrate  the fundamental benefits of Thompson Sampling over $\varepsilon$-greedy and Boltzmann exploration strategies  using simplified examples. In Table~\ref{table:reasons}, we list the three strategies and their properties. 

%%
%\begin{figure*}[t]
%  \begin{minipage}[]{0.5\textwidth}
%	 \centering
%% \includegraphics[width=1.\linewidth]{Fig/secondbest.png}
%\includegraphics[width=0.9\linewidth]{Fig/low-action2.pdf}\\
%(a)
%  \end{minipage}%\hfill
%  \begin{minipage}{0.5\textwidth}
%     \centering
%	 \includegraphics[width=0.8\linewidth]{Fig/low-action.pdf}\\
%% 	 \includegraphics[width=1.\linewidth]{Fig/lowestpicked.png}
%     (b)
%  \end{minipage}
%%   \begin{minipage}{0.33\textwidth}
%%      \centering
%%      \vspace{-0.8cm}
%% \includegraphics[width=0.80\linewidth]{Fig/maze1.eps}
%% (c)
%%   \end{minipage}
%   \caption{Thompson Sampling vs $\varepsilon$-greedy and Boltzmann exploration. $(a)$ $\varepsilon$-greedy is wasteful since it assigns uniform probability to explore over $5$ and $6$, which are obviously sub-optimal when the uncertainty estimates are available. Boltzmann exploration randomizes over actions even if the optimal action is identifies. (b) Boltzmann exploration does not incorporate uncertainties over the estimated action-values and chooses actions 5 and 6 with similar probabilities while action 6 is significantly more uncertain. Thomson Sampling is a simple remedy to all these issues. 
%}
%\label{fig:uncertainty}
%\end{figure*}
%%

$\varepsilon$-greedy is among the simplest exploration-exploitation strategies and it is uniformly random over all the non-greedy actions. Boltzmann exploration is an intermediate strategy since it uses the estimated $Q$ function to sample from action space. However, it does not maintain uncertainties over the $Q$ function estimation. In contrast, Thompson sampling incorporates the $Q$ estimate as well as the uncertainties in the estimation and utilizes the most information for exploration-exploitation strategy.  

Consider the example in Figure~\ref{fig:uncertainty}(a) with our current estimates and uncertainties of the $Q$ function over different actions.   $\varepsilon$-greedy is not compelling since it assigns uniform probability to explore over $5$ and $6$, which are sub-optimal when the uncertainty estimates are available. In this setting, a possible remedy is Boltzmann exploration since it assigns lower probability to actions $5$ and $6$ but randomizes with almost the same probabilities over the remaining actions.

%
\begin{figure}[h]
  \begin{minipage}[]{0.27\textwidth}
	 \centering
% \includegraphics[width=1.\linewidth]{Fig/secondbest.png}
     \hspace*{-0.4cm}
\includegraphics[trim={0cm 0 0 0},clip,height=.9\linewidth]{Fig/low-action2-blue.eps}\\
     \hspace*{-.0cm}(a)
  \end{minipage}%\hfill
  \begin{minipage}{0.27\textwidth}
     \centering
     \hspace*{-0.5cm}
	 \includegraphics[trim={4cm 0 0 0},clip,height=.9\linewidth]{Fig/low-action-blue.eps}\\
% 	 \includegraphics[width=1.\linewidth]{Fig/lowestpicked.png}
     \hspace*{-1.5cm}     (b)
  \end{minipage}
%   \begin{minipage}{0.33\textwidth}
%      \centering
%      \vspace{-0.8cm}
% \includegraphics[width=0.80\linewidth]{Fig/maze1.eps}
% (c)
%   \end{minipage}
   \caption{Thompson Sampling vs $\varepsilon$-greedy and Boltzmann exploration. $(a)$ $\varepsilon$-greedy is wasteful since it assigns uniform probability to explore over $5$ and $6$, which are obviously sub-optimal when the uncertainty estimates are available. Boltzmann exploration randomizes over actions even if the optimal action is identifies. (b) Boltzmann exploration does not incorporate uncertainties over the estimated action-values and chooses actions 5 and 6 with similar probabilities while action 6 is significantly more uncertain. Thomson Sampling is a simple remedy to all these issues. 
}
\label{fig:uncertainty}
\end{figure}


 
 
However, Boltzmann exploration is sub-optimal in settings where there is high uncertainty. For example if the current $Q$ estimate is according to Figure ~\ref{fig:uncertainty}(b), then Boltzmann exploration assigns almost equal probability to actions $5$ and $6$, even though action $6$ has much higher uncertainty and needs to be explored more. 

Thus, both  $\varepsilon$-greedy and Boltzmann exploration strategies are sub-optimal since they do not maintain an uncertainty estimate over the $Q$ estimation. In contrast, Thompson sampling uses both estimated $Q$ function and its uncertainty estimates to carry out a more efficient exploration.

%throw way a significant portion of information for their exploration. On the other hand, Thompson Sampling deploys all this information in order to design a strategic exploration-exploration trade-off. Thompson sampling avoids wasting its sampling budget by eluding to sample the actions which are already understood to be sub-optimal. Therefore it gains significantly better sample complexity. Moreover, since it collects a desirably more useful set of experience, for replay-buffer based DRL where we have a limited budget of storing experiences as well as limited capacity for $Q$-functions, having useful samples helps to approximate the $Q$-value better.


% approaches  just care about the greedy action ad
% In this section, we enumerate a few benefits of \TS which use of both estimated Q value and  over $\varepsilon$-greedy and Boltzmann exploration. We show how \TS exploit both the estimated and the uncertainties of returns to design a randomized exploration while $\varepsilon-$greedy disregards all these useful information and Boltzmann exploration disregards the estimation uncertainty for exploration. 



==> Sections/alter-11-Bayesian.tex <==
\subsection{Bayesian Regret of Alg.~\ref{alg:psrl}}\label{sec:proof}
The analysis developed in the previous section, up to some minor modification, e.g., change of strategy to \PSRL,  directly applies to Bayesian regret bound, with a farther expectation over models.


When there is a prior over the $\omega^*$  the expected Bayesian regret might be the target of the study. 
\begin{align*}
\textbf{BayesReg}_T:&=\E\left[\sum_t^T \left[V^{\omega^*}_{\pi^*}-V^{\omega^*}_{\pi_t}\right]\right]\\
&\E\left[\sum_t^T\left[ V^{\omega^*}_{\pi^*}-V^{\omega^*}_{\pi_t}\big|\mathcal{H}_t\right]\right]
\end{align*}
Here $\mathcal{H}_t$ is a multivariate random sequence which indicates history at the beginning of episode $t$ and  $\pi_t$ is the policy following \PSRL. For the remaining $\pi_t$ denotes the \PSRL policy. As it mentioned in the Alg.~\ref{alg:psrl}, at the beginning of an episode, we draw $\omega_t$ for the posterior and the corresponding policy is 
\begin{align*}
    \pi_t(X_t^h):=\arg\max_{a\in\A}\phi(X_t^h,a)^\top\omega_t
\end{align*}
Condition on the history $\mathcal{H}_t$, samples by following the agent policy $\pi_t'$ for each episode $t'\leq t$, similar to previous section we estimate the $\wh \omega_t$ as follows; 
\begin{align*}
\wh\omega_t:= \left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\mathbf{\wb R}_i\right)
\end{align*}
Lemma~\ref{lem:conf} states that under event $\Theta_T$, $\|\wh\omega_t-\omega^*\|_{\wo\chi_t}\leq\theta_t(\delta)$. Conditioned on $\mathcal{H}_t$, the $\omega_t$ and $\omega^*$ are equally distributed, then we have
\begin{align*}
 \E\left[V^{\wt\omega_t(\pi^*)}_{\pi^*}\big|\mathcal{H}_t\right]=\E\left[ V^{\wt\omega_t(\pi_t)}_{\pi_t}\big|\mathcal{H}_t\right]   
\end{align*}
Therefore, under event $\Theta_T$ holds for all $\omega^*$ we have

\begin{align*}
\textbf{BayesReg}_T:&=\sum_t^T\E\left[\underbrace{V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(X_t^1)}_{\Delta_t^{h=1}}|\mathcal{H}_t\right]\\
&=\sum_t^T\E\left[V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)+V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(X_t^1)|\mathcal{H}_t\right]\\
&=\sum_t^T\E\left[ V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\omega^*}_{\pi_t}(X_t^1)+\underbrace{V^{\omega^*}_{\pi^*}(X_t^1)-V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)}_\text{$\leq 0$}|\mathcal{H}_t\right]\\
% &=\sum_t^T V^{\wt\omega_t}_{\pi_t}(x_t^1)-V^{\omega^*}_{\pi_t}(x_t^1)%=\sum_t^T\phi(x_t^1,\pi_t(x_t^1))^\top \left(\wt\omega_t-\omega^*\right)
\end{align*}
Resulting in 
\begin{align*}
\textbf{BayesReg}_T&\leq\sum_t^T\E\left[ V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\omega^*}_{\pi_t}(X_t^1)|\mathcal{H}_t\right]
%=\sum_t^T\phi(x_t^1,\pi_t(x_t^1))^\top \left(\wt\omega_t-\omega^*\right)
\end{align*}

Similar to optimism and defining $V^{\omega}_{\pi}(X_t^1,\ldots, X_t^{h'};h:\pi')$ accomponeid with Eq.\ref{eq:Bayesian_model} we have;
\begin{align*}
\textbf{BayesReg}_T&\leq\E\left[\sum_t^T \left[V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\omega^*}_{\pi_t}(X_t^1)|\mathcal{H}_t\right]\right]\\
&=\E\left[\sum_t^T \left[V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)+V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^1)|\mathcal{H}_t\right]\right]\\
&\leq\E\left[\sum_t^T\left[ \phi(X_t^1,\pi_t(X_t^1))^\top\wt\omega_t(\pi_t)-\phi(X_t^1,\pi_t(X_t^1))^\top\omega^*+V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^1)|\mathcal{H}_t\right]\right]\\
&=\E\left[\sum_t^T \left[\phi(X_t^1,\pi_t(X_t^1))^\top\left(\wt\omega_t(\pi_t)-\omega^*\right)+\underbrace{V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^1)}_{(\Delta_t^{h=2})}|\mathcal{H}_t\right]\right]
%=\sum_t^T\phi(x_t^1,\pi_t(x_t^1))^\top \left(\wt\omega_t-\omega^*\right)
\end{align*}
% Given the generative model in Eq.\ref{eq:Bayesian_model} we have
% \begin{align*}
% \textbf{BayesReg}_T&\leq\E\left[\sum_t^T V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)+V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^1)|\omega^*\right]\\
% &\leq\E\left[\sum_t^T \phi(X_t^1,\pi_t(X_t^1))^\top\wt\omega_t(\pi_t)-\phi(X_t^1,\pi_t(X_t^1))^\top\omega^*+V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^1)|\omega^*\right]\\
% &=\E\left[\sum_t^T \phi(X_t^1,\pi_t(X_t^1))^\top\left(\wt\omega_t(\pi_t)-\omega^*\right)+\underbrace{V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^1)}_{(\Delta_t^{h=2})}|\omega^*\right]
% %=\sum_t^T\phi(x_t^1,\pi_t(x_t^1))^\top \left(\wt\omega_t-\omega^*\right)
% \end{align*}
% V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^1)
For $\Delta_t^{h=2}$ we deploy the similar decomposition and upper bound as $\Delta_t^{h=1}$
\begin{align*}
\Delta_t^2:=V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^1)
\end{align*}
Since for both of $V^{\omega^*}_{\pi_t}(X_t^1;1:\pi^*)$ and $V^{\omega^*}_{\pi_t}(X_t^1)$ we follow the same distribution over policies and models for 1 time step, the reward at the first time step has the same distribution, therefore we have;
\begin{align*}
\Delta_t^{h=2}&=E\left[V^{\omega^*}_{\pi_t}(X_t^2;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^2)|X_t^1,\mathcal{H}_t\right]
\end{align*}
rustling in 
\begin{align*}
\Delta_t^{h=2}&=E\left[V^{\omega^*}_{\pi_t}(X_t^2;1:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^2)|X_t^1,\mathcal{H}_t\right]\\
&\leq\E\left[\phi(X_t^2,\pi_t(X_t^2))^\top\left(\wt\omega_t(\pi_t)-\omega^*\right)+\underbrace{V^{\omega^*}_{\pi_t}(X_t^2;2:\pi^*)-V^{\omega^*}_{\pi_t}(X_t^2)}_{(\Delta_t^{h=3})}|X_t^1,\mathcal{H}_t\right]
\end{align*}
Similarly we can defined $\Delta_t^{h=3}, \ldots \Delta_t^{h=H}$. The condition on $\mathcal{H}_t$ was required to come up with the mentioned decomposition through $\Delta_t^{h}$ and it is not needed anymore, therefore;



\begin{align}\label{eq:bayesunit}
\textbf{BayesReg}_T&\leq\E\left[\sum_t^T\sum_h^H \phi(X_t^h,\pi_t(X_t^h))^\top\left(\wt\omega_t(\pi_t)-\omega^*\right)\right]\nonumber\\
&=\sum_t^T\E\left[\mathbbm{1}^\top\mathbf{\Phi}_t\left(\wt\omega_t(\pi_t)-\omega^*\right)\right]\nonumber\\
&=\E\left[\sum_t^T\mathbbm{1}^\top\mathbf{\Phi}_t\wo\chi_{t-1}^{-1/2}\wo\chi_{t-1}^{1/2}\left(\wt\omega_t(\pi_t)-\omega^*\right)\right]\nonumber\\
&\leq \E\left[\sqrt{H}\sum_t^T \|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}\|\wt\omega_t(\pi_t)-\omega^*\|_{\wo\chi_{t-1}}\right]\nonumber\\
&\leq \E\left[\sqrt{H} \sum_t^T\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}2\theta_{t-1}(\delta)\right]
\end{align}
% Where $\delta$ is the probability that we desire the event $\Theta$ hold for a specific $\omega^*$.
Again similar to optimism we have the maximum expected cumulative reward condition on states of a episode is at most $1$, we have;
\begin{align*}
\textbf{BayesReg}_T&\leq\sqrt{H}\E\left[\sum_t^T \min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}2\theta_{t-1}(\delta),1\rbrace\right]\\
&\leq\sqrt{H}\E\left[\sum_t^T\sum_h^H2\theta_{t-1}(\delta) \min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}},1\rbrace\right]\\
\end{align*}


Moreover, at time $T$, we can use Jensen's inequality, exploit the fact that $\theta_t(\delta)$ is an increasing function of $t$ and have

\begin{align}\label{eq:regpsrl}
\textbf{BayesReg}_T&\leq2\E\left[\sqrt{TH\theta_{T}(\delta)^2\sum_t^T \min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}},1\rbrace}\right]\nonumber\\
&\leq2 
\left(\sigma\sqrt{2
\log\left(1/\delta\right)
+d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\E\left[\sqrt{TH\sum_t^T\min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}},1\rbrace}\right]\nonumber\\
&\leq
2\left(\sigma\sqrt{2
\log\left(1/\delta\right)
+d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2TH d\log(\lambda + TL^2/d)}
\end{align}
% (\omega^*)
% We set $\delta = \delta P(\omega^*)/P_{\max}$, with $P(\cdot)$ represents the prior distribution on $\omega^*$ and $P_{\max}:=\max\lbrace\max_{\omega*}P(\omega^*),1\rbrace$. 
% We have the following by Cauchy Schwarz
% \begin{align*}
%     \E\left[\sqrt{2
% \log\left(1/\delta\right)
% +d\log\left(1+TL^2/\lambda\right)}\right]
% \leq\sqrt{2/P_{\max}}\mathbbm{H}+\sqrt{2
% \log\left(1/\delta\right)
% +d\log\left(1+TL^2/\lambda\right)}
% \end{align*}
% where $\mathbbm{H}$ is the differential entropy of the prior. Substituting the RHS of Eq.~\ref{eq:xx} into Eq.~\ref{eq:BR1}, we get 
% Therefore we can restate the regret as 

% \begin{align}\label{eq:regpsrl}
% \textbf{BayesReg}_T\leq 
% 2\left(\sqrt{2/P_{\max}}\mathbbm{H}\sigma+\sigma\sqrt{2
% \log\left(1/\delta\right)
% +d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2TH d\log(\lambda + TL^2/d)}
% \end{align}
% \begin{align}\label{eq:regpsrl}
% \textbf{BayesReg}_T\leq 
% 2\left(\sigma\sqrt{2
% \log\left(1/\delta\right)
% +d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2TH d\log(\lambda + TL^2/d)}
% \end{align}
Under event $\Theta_T$ which holds with probability at least $1-\delta$. If we set $\delta=1/T$ then the probability that the event $\Theta$ holds is $1-1/T$ and we get regret of at most the RHS of Eq.~\ref{eq:regpsrl}, otherwise with probability at most $1/T$ we get maximum regret of $T$, therefore 
% \begin{align*}
% \textbf{BayesReg}_T1+\leq 
% 2\left(\sqrt{2/P_{\max}}\mathbbm{H}\sigma+\sigma\sqrt{2
% \log\left(T\right)
% +d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2TH d\log(\lambda + TL^2/d)}
% \end{align*}
\begin{align*}
\textbf{BayesReg}_T\leq 1+
2\left(\sigma\sqrt{2
\log\left(T\right)
+d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2TH d\log(\lambda + TL^2/d)}
\end{align*}
and theorem statement follows.

==> Sections/alter-12-Lemmas.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discount factor}\label{sub:discount}

Through the analysis of the theorems~\ref{Thm:BR} and~\ref{Thm:frequentist} we studied the regret upper bounds for undiscounted reward MDP{}s when $\gamma=1$. If we consider the problem expression as follows
\begin{align*}
\mathbf{\wb R}_t:=\Psi \mathbf{R}_t~~~\wb\nu_t:=\Psi\nu_t
\end{align*}
the parameter $\wb\nu_t$ for a general matrix $\Psi$ represent the stochasticity of the return under any discount factor $0\leq\gamma\leq 1$. Under the general discount factor, the Assumption~\ref{asm:subgaussian} describes the sub-Gaussian characteristics of $\wb\nu_t$. Moreover under discounted return, the value function represent the expectation of the discounted return, resulting in a potentially smaller $L_\omega$. Furthermore, in the decompositions derived in the Eqs.~\ref{eq:onesnorm} and ~\ref{eq:bayesunit} regarding $\Delta_t^h$ we require to aggregate the regret while discounting the per step regrets. It means we replace $\mathbbm{1}$ with
$[1,\gamma,\gamma^2,\ldots,\gamma^{H-1}]^\top$ in those equations. Consequently, instead of considering the $\|\mathbbm{1}\|_2$ to upper bound the regrets, we are interested in the discounted returns and consider $\|[1,\gamma,\gamma^2,\ldots,\gamma^{H-1}]\|_2$ to come up with the corresponding upper bounds and replace $\sqrt{H}$ in the final statements of the theorems~\ref{Thm:BR} and~\ref{Thm:frequentist} with a discount factor dependent and smaller value $\|[1,\gamma,\gamma^2,\ldots,\gamma^{H-1}]\|_2$.


\subsection{Proof of Lemmas}

\begin{lemma}\label{lem:M_t}
Let $\alpha\in\R^d$ be be an arbitrary vector and for any $t\geq0$ define
\begin{align*}
M_t^\alpha :=\exp\left(\sum_i^t\left[\frac{\alpha^\top \mathbf{\Phi}_i^\top\Psi'\nu_i}{\sigma}-\frac{1}{2}\|\Psi^{-1}\mathbf{\Phi_i}\alpha\|^2_2\right]\right)
\end{align*}
Then, for a stopping time under the filtration $\{\F_t\}_{t=0}^\infty$, $M_\tau^\lambda\leq 1$.
\end{lemma}



\begin{proof}~Lemma~\ref{lem:M_t}
We first show that $\{M_t^\alpha\}_{t=0}^\infty$ is a supermartingale sequence. Let
\begin{align*}
D_i^\alpha = \exp\left(\frac{\alpha^\top \mathbf{\Phi}_i^\top\Psi'\nu_i}{\sigma}-\frac{1}{2}\|\Psi^{-1}\mathbf{\Phi_i}\alpha\|^2_2\right)
\end{align*}
Therefore, we can rewrite $\E\left[M^\alpha_t\right]$ as follows:
\begin{align*}
\E\left[M_t^\alpha|\F_{t-1}\right] = \E\left[D_1^\alpha\ldots D_{t-1}^\alpha D_{t}^\alpha|\F_{t-1}\right] = D_1^\alpha\ldots D_{t-1}^\alpha\E\left[ D_{t}^\alpha|\F_{t-1}\right]\leq M_{t-1}^\alpha
\end{align*}
The last inequality follows since $\E\left[ D_{t}^\alpha|\F_{t-1}\right]\leq 1$ due to Assumption~\ref{asm:subgaussian}, therefore since for the first time step $\E\left[M_1^\alpha\right]\leq 1$, then $\E\left[M_t^\alpha\right]\leq 1$. For a stopping time $\tau$, Define a variable $\wo{M}_t^\alpha = M_{\min\{t,\tau\}}^\alpha$ and since $\E\left[M_\tau^\alpha\right]= \E\left[\lim\inf_{t\rightarrow\infty}\wo{M}_t^\alpha\right]\leq \lim\inf_{t\rightarrow \infty}\E\left[\wo{M}_t^\alpha\right]\leq 1$, therefore the Lemma~\ref{lem:M_t} holds.
\end{proof}

% Let's defined the following quantities for self-normalized processes;
% \begin{align*}
% S_t := \sum_i^t \mathbf{\Phi}_i^\top\wb\nu_i, ~~~~~ \chi_t := \sum_{i=0}^t  \mathbf{\Phi}_i^\top\mathbf{\Phi}_i, ~~~~~ \wo\chi_t = \chi_t+\wt\chi
% \end{align*}
% where $\wt\chi$ is a ridge regularization matrix and usually is equal to $\lambda I$.
\begin{lemma} \label{lem:self}[Extension to Self-normalized bound in \cite{abbasi-yadkori2011improved}] For a stopping time $\tau$ and filtration $\{\F_t\}_{t=0}^\infty$, with probability at least $1-\delta$
\begin{align*}
\|S_\tau\|_{\wo\chi_\tau^{-1}}^2\leq 2\sigma^2\log(\frac{\det\left(\wo\chi_t\right)^{1/2}\det(\wt\chi)^{-1/2}}{\delta})
\end{align*}
\end{lemma}
\begin{proof}~of Lemma~\ref{lem:self}.
Given the definition of the parameters of self-normalized process, we can rewrite $M_t^\alpha$ as follows;
\begin{align*}
M_t^\alpha = \exp\left(\frac{\alpha^\top S_t}{\sigma}-\frac{1}{2}\|\alpha\|_{\chi_t}\right)
\end{align*}
Consider $\Omega$ as a Gaussian random vector and $f(\Omega=\alpha)$ denotes the density with covariance matrix of $\wo \chi^{-1}$. Define $M_t:=\E\left[M_t^\Omega|\F_\infty\right]$. Therefore we have $\E\left[M_t\right]=\E\left[\E\left[M_t^\Omega|\Omega\right]\right]\leq 1$. Therefore
\begin{align*}
M_t=&\int_{\Re^d}\exp\left(\frac{\alpha^\top S_t}{\sigma}-\frac{1}{2}\|\alpha\|_{\chi_t}\right)f(\alpha)d\alpha\\
%
=&\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\frac{1}{2}\|S_t/\sigma\|^2_{\chi_t^{-1}}\right)f(\alpha)d\alpha\\
%
=&\sqrt{\frac{\det\left(\wt\chi\right)}{\left(2\pi\right)^d}}\exp\left(\frac{1}{2}\|S_t/\sigma\|_{\chi_t^{-1}}\right)\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\frac{1}{2}\|\alpha\|^2_{\wt\chi}\right)d\alpha
\end{align*}
Since $\chi_t$ and $\wt\chi$ are positive semi definite and positive definite respectively, we have 
\begin{align*}
\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\|\alpha\|^2_{\wt\chi}&= \|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}+\|\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}-\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}\\
&=\|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}+\|\S_t/\sigma\|^2_{\chi_t^{-1}}-\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}
\end{align*}
Therefore, 
\begin{align*}
M_t=&\sqrt{\frac{\det\left(\wt\chi\right)}{\left(2\pi\right)^d}}\exp\left(\frac{1}{2}\|S_t/\sigma\|_{\left(\wt\chi+\chi_t\right)^{-1}}\right)\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}\right)d\alpha\\
=&\left(\frac{\det\left(\wt\chi\right)}{\det\left(\wt\chi+\chi_t\right)}\right)^{1/2}\exp\left(\frac{1}{2}\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}\right)
\end{align*}
Since $\E\left[M_\tau\right]\leq 1$ we have
\begin{align*}
\Prob\left(\|S_\tau\|^2_{\left(\wt\chi+\chi_\tau\right)^{-1}}\leq 2\sigma\log\left(\frac{\det\left(\wt\chi+\chi_\tau\right)^{1/2}}{\delta\det\left(\wt\chi\right)^{1/2}}\right)\right)
\leq \frac{\E\left[\exp\left(\frac{1}{2}\|S_\tau/\sigma\|^2_{\left(\wt\chi+\chi_\tau\right)^{-1}}\right)\right]}{\left(\frac{\det\left(\wt\chi+\chi_\tau\right)}{\delta\det\left(\wt\chi\right)}\right)^{1/2}}\leq \delta
\end{align*}
Where the Markov inequality is deployed for the final step. 
The stopping is considered to be the time step as the first time in the sequence when the concentration in the Lemma~\ref{lem:self} does not hold. 
\end{proof}





%%%%%%%%
\begin{proof}[Proof of Lemma \ref{lem:conf}]
Given the estimator $\wh\omega_t$ we have the following:
\begin{align*}
\wh\omega_t&=\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\left(\Psi^{-1}\mathbf{\Phi}_i\omega^* + \nu_i\right)\right)\\
&=\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\\
&+ \left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)\omega^*\\
&-\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\omega^*\\
\end{align*}
therefore, for any vector $\zeta\in\Re^d$
\begin{align*}
\zeta^\top\wh\omega_t-\zeta^\top\omega^*&=\zeta^\top\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\\
&-\zeta^\top\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\omega^*
\end{align*}
As a results, 
applying Cauchy-Schwarz inequality and inequalities $\|\omega^*\|_{\wo\chi_t^{-1}}\leq \frac{1}{\lambda\left(\wo\chi_t\right)}\|\omega^*\|_2\leq \frac{1}{\lambda}\|\omega^*\|_2$ we get
\begin{align*}
|\zeta^\top\wh\omega_t-\zeta^\top\omega^*|&\leq\|\zeta\|_{\wo\chi_t^{-1}}\|\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\|_{\wo\chi_t^{-1}}+\lambda\|\zeta\|_{\wo\chi_t^{-1}}\|\omega^*\|_{\wo\chi_t^{-1}}\\
&\leq \|\zeta\|_{\wo\chi_t^{-1}}\left(\|\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\|_{\wo\chi_t^{-1}}+\lambda^{1/2}\|\omega^*\|_2\right)
\end{align*}
where applying self normalized Lemma \ref{lem:self}, with probability at least $1-\delta$
\begin{align*}
|\zeta^\top\wh\omega_t-\zeta^\top\omega^*|\leq \|\zeta\|_{\wo\chi_t^{-1}}\left(2\sigma\log\left(\frac{\det\left(\wo\chi_t\right)^{1/2}}{\delta\det\left(\wt\chi\right)^{1/2}}\right)+\lambda^{1/2}L_\omega\right)
\end{align*}
hold for any $\zeta$. By plugging in $\zeta=\wo\chi_t\left(\wh\omega_t-\omega^*\right)$ %we get the statement in the Lemma \ref{lem:conf}.
we get the following;
\begin{align*}
\|\wh\omega_t-\omega^*\|_{\wo\chi_t}\leq\theta_t(\delta)= \sigma\sqrt{2\log\left(\frac{\det(\wo\chi_t)^{1/2}\det(\lambda I)^{-1/2}}{\delta}\right)}+\lambda^{1/2}L_\omega
\end{align*}
The $\det(\wo\chi_t)$ can be written as $\det(\wo\chi_t)=\prod_j^d\alpha_j$ therefore, $trace(\wo\chi_t)=\sum_j^d\alpha_j$. We also know that;
\begin{align*}
    (\prod_j^d\alpha_j)^{1/d}\leq \frac{\sum_j^d\alpha_j}{d}
\end{align*}
A matrix extension to Lemma 10 and 11 in \cite{abbasi-yadkori2011improved} results in  $\det(\wo\chi_t)\leq \left(\frac{trace(\wo\chi_t)}{d}\right)^d$ while we have $trace(\wo\chi_t)=trace(\lambda I)+trace(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i)\leq d\lambda+tL$, 
\begin{align}\label{eq:deter}
    \det(\wo\chi_t)\leq \left(\frac{d\lambda+tL}{d}\right)^d
\end{align}


therefore the main statement of Lemma \ref{lem:conf} goes through.
\end{proof}



% \eb{Wait, I'm confused. I thought we just proved Lemma 3. And the below is not stated as a lemma. Could you clarify please?}

% \begin{lemma}[Determinant inequality]
% For a matrix problem in Eq.~\ref{eq:Bayesian_model}, given a sequence of $\lbrace\mathbf{\Phi}_i,\mathbf{R}_i\rbrace_{i=1}^{t}$, and under $trace{\mathbf{\Phi}(\cdot)\mathbf{\Phi}(\cdot)^\top}\leq L$  we have:
% \begin{align*}
% \det\left(\wo\chi_t\right)\leq (\lambda+tL^2/d)^d\quad,\quad \sum
% \end{align*}
% \end{lemma}


% \textbf{BayesReg}_T:&=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[\phi(x_t^1,\pi_t(x_t^1))^\top \omega(\pi_t)-\phi(x_t^1,\pi_t(x_t^1))^\top \omega^* \big|\mathcal{H}_t\right]\right]\\
% &\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[\phi(x_t^1,\pi_t(x_t^1))^\top \left(\wt\omega_t(\pi_t)-\omega^*\right) \big|\mathcal{H}_t\right]\right]
% \end{align*}







\begin{proof}~Lemma~\ref{lemma:DeterminantLemma}
We have the following for the determinant of $\det\left(\wo\chi_T\right)$

\begin{align*}
\det\left(\wo\chi_T\right)&=\det\left(\wo\chi_{T-1}+\mathbf{\Phi}_T^\top\Psi'\Psi^{-1}\mathbf{\Phi}_T\right)\\
&=\det\left(I_H+\mathbf{\Phi}_T\wo\chi_{T-1}^{-1}\mathbf{\Phi}_T^\top\right)\det\left(\wo\chi_{T-1}\right)\\
&=\prod_t^T\det\left(I_H+\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top\right)\det\left(\wt\chi\right)
\end{align*}
From linear algebra, and given a time step $t$, we define the characteristic polynomial of the matrix $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ as;
\begin{align*}
    CP_t(\wb\lambda)=\det(\wb\lambda I_H-\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top).
\end{align*}
% $CP_t(\wb\lambda)=\det(\wb\lambda I_H-\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top)$. 
If the set $\lbrace\lambda_1,\lambda_2,\ldots,\lambda_d\rbrace$ represent the eigenvalues of $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ where $\lambda_i\geq\lambda_j$ if $i\geq j$, one can rewrite $CP_t(\wb\lambda)$ as follows;
\begin{align*}
    CP(\wb\lambda) = (\wb\lambda-\lambda_1)(\wb\lambda-\lambda_2)\cdots (\wb\lambda-\lambda_H)
\end{align*} 
Now by adding the matrix $I_H$ to $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$, we get $CP_t'(\wb\lambda)=\det(\wb\lambda I_H-I_H-\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top)$, therefore;
\begin{align*}
    CP_t'(\wb\lambda) = (\wb\lambda-1-\lambda_1)(\wb\lambda-1-\lambda_2)\cdots (\wb\lambda-1-\lambda_H)
\end{align*} 
and the eigenvalues of $I_H+\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ are shifted eigenvalues of $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ by $+1$, i.e. $\lbrace\lambda_1+1,\lambda_2+1,\ldots,\lambda_d+1\rbrace$. Since $\xi^\top\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top\xi=\left(\mathbf{\Phi}{\wo\chi_t^{-1/2}}^\top\xi\right)^\top\left(\mathbf{\Phi}{\wo\chi_t^{-1/2}}^\top\xi\right)$ all the eigenvalues $\lbrace\lambda_1,\lambda_2,\ldots,\lambda_d\rbrace$ are non-negative. As a results,
\begin{align*}
    \det\left(I_H+\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top\right)\geq \left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)
\end{align*}
As a consequence; 
\begin{align*}
    \det\left(\wo\chi_T\right)\geq\det\left(\wt\chi\right) \prod_t^T\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}\right)
\end{align*}
Moreover we have
% \begin{align}
% \sum_t^T\log\left(1+\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\right)\leq \sum_t^T\log\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)
% \end{align}

\begin{align}%\label{eq:xx}
2\sum_t^T\log\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)\leq 2\left(\log\left(\det\left(\wo\chi_T\right)\right)-\log\left(\det\left(\wt\chi\right)\right)\right)\leq 2 d\log(\lambda + TL^2/d)
\end{align}

and the statement follows.



\end{proof}











==> Sections/diagram.tex <==
% Double Arrows a la Chef
% Author: Dominik Haumann


% for double arrows a la chef
% adapt line thickness and line width, if needed
\tikzstyle{vecArrow} = [thick, decoration={markings,mark=at position
   1 with {\arrow[semithick]{open triangle 60}}},
   double distance=1.4pt, shorten >= 5.5pt,
   preaction = {decorate},
   postaction = {draw,line width=1.4pt, white,shorten >= 4.5pt}]
\tikzstyle{innerWhite} = [semithick, white,line width=1.4pt, shorten >= 10.5pt]



\begin{tikzpicture}[thick]
  \node[draw,rectangle] (a) {Estimate $\wt\omega_t$};
  \node[inner sep=0,minimum size=0,right of=a] (k) {}; % invisible node
  \node[draw,rectangle,right of=k] (b) {B};
  \node[draw,rectangle,below of=a] (c) {C};

  % 1st pass: draw arrows
  \draw[vecArrow] (a) to (b);
  \draw[vecArrow] (k) |- (c);

  % 2nd pass: copy all from 1st pass, and replace vecArrow with innerWhite
  \draw[innerWhite] (a) to (b);
  \draw[innerWhite] (k) |- (c);

  % Note: If you have no branches, the 2nd pass is not needed
\end{tikzpicture}


==> Sections/old-10-Theory-H-dependent.tex <==
\section{Bayesian Regret, Proof of Theorem \ref{Thm:BR}}\label{sec:proof}
Let's consider the following linear model over the $Q$ functions and returns for episodic MDPs with episode length of $H$. (We consider the discount factor to be any number $0\leq \gamma\leq 1$)



\begin{equation}\label{eq:Bayesian_model}
\Psi\mathbf{R} = \mathbf{\Phi}(x^{\{1:H\}},a^{\{1:H\}})\omega +\Psi \nu(x^{\{1:H\}},a^{\{1:H\}})~,~~ \textit{where}~,~\Psi:=\left[
  \begin{tabular}{ccccc}
  1 & $\gamma$ & $\gamma^2$ &$\ldots$ & $\gamma^{H-1}$\\
  0 & 1 & $\gamma$ &  $\ldots$ & $\gamma^{H-2}$\\
  0 & 0 & $1$ & $\ldots$ &$\vdots$ \\
  $\vdots$ & $\ldots$ & $\ldots$& $\ldots$ & $\vdots$\\
  $0$ & $\ldots$ & $\ldots$& $\ldots$ & 1
  \end{tabular}
\right]
\end{equation}
Where the Q function is a linear function of $\phi(x,a)\in \R^d$, i.e. $Q(x,a):=\phi(x,a)^\top\omega$. In order to study the most general setting, we also represent actions through the same feature representation. The vector $\mathbf{R}\in \Re^H$ is the random vector of rewards in a episode. The matrix $\mathbf{\Phi}(x^{\{1:H\}},a^{\{1:H\}})\in\Re^{H\times d}$ is a row-wised concatenation of sequence of state-action features, $\phi(x,a)$ under a given policy, also any instance of the feature representing matrix,  $trace\left(\mathbf{\Phi}(x^{\{1:H\}},a^{\{1:H\}})\mathbf{\Phi}(x^{\{1:H\}},a^{\{1:H\}})^\top\right)\leq L~,~\textit{for any}x^{\{1:H\}},a^{\{1:H\}} $. The vector $\nu(x^{\{1:H\}},a^{\{1:H\}})\in\Re^H$% \sim \N(0,\Sigma_\epsilon(x_{\{1:H\}},a_{\{1:H\}))$
is a state-action dependent noise vector where, for any $h'$, the noises after time step $h'$, $\nu^{h=i\geq h'}$, are independent from the noises before time step $h'$, $\nu^{h=i< h'}$ condition on $(x^h,a^h)$, the state action pair at time step $h$. Moreover, since the underlying model of environment is assumed to be an MDP, the noise at time step $h$, $\nu^h$ models the induces noise by stochasticity of transition distribution to state $x^h$, i.e. $f(x^h|x^{h-1},a^{h-1})$, and the stochasticity of reward at time step $h$, i.e. $r(x^h,a^h)$.
In the Bayesian approach, we consider a Gaussian prior over the parameter vector $\omega\sim\N(0,\lambda I)$, then exploit the samples to compute the posterior. After computing the posterior at time $t$ we sample a vector $\omega_t$, then follow the policy induced by $\omega_t$, i.e. $\pi_t$. We then collect the resulting trajectory to update the posterior and the policy for next episode. 

In the following, we show that, given the true underlying model has parameter $\omega^*$, after $T$ episodes of following \TS, the estimated $\hat{b}_t$ concentrates around its true value $\omega^*$. The main body of the following analyses on concentration of measure is a matrix extension of  contextual linear bandit analyses \cite{abbasi-yadkori2011improved,chu2011contextual,li2010contextual,rusmevichientong2010linearly,dani2008stochastic} and self normalized processes\citep{de2004self}. Our regret analysis extends prior analysis in frequentist and Bayesian regret literature \cite{osband2013more,jaksch2010near}.

In order to provide more intuition on the model, we can exploit the property of the matrix $\Psi$ where
\begin{align*}
\Psi^{-1}=\left[
  \begin{tabular}{ccccc}
  1 & $-\gamma$ & 0 &$\ldots$ & 0\\
  0 & 1 & -$\gamma$ &  $\ldots$ & 0\\
  0 & 0 & $1$ & $\ldots$ &$\vdots$ \\
  $\vdots$ & $\ldots$ & $\ldots$& $\ldots$ & $\vdots$\\
  $0$ & $\ldots$ & $\ldots$& $\ldots$ & 1
  \end{tabular}
\right]
\end{align*}
and rewrite Eq.~\ref{eq:Bayesian_model} as follows:

\begin{equation}
\mathbf{R}_t = \Psi^{-1}\mathbf{\Phi}_t\omega + \nu_t
\end{equation}
We denote $\Psi':={\Psi^{-1}}^\top$. Let's restate the Eq.~\ref{eq:Bayesian_model} in its abtract way;
\begin{equation}
\mathbf{\wb R}_t:=\Psi \mathbf{R}_t=\mathbf{\Phi}_t\omega + \wb\nu_t~,~~~\textit{where}~~~\wb\nu_t:=\Psi\nu_t
\end{equation}
% \eb{This is a bit unclear. Is this an assumption on the model of the environment, or a particular representation/decomposition that is independent of the domain?}

\begin{assumption}[Sub-Gaussian random vector \citep{hsu2012tail}]\label{asm:subgaussian}
The noise model at time $t$, conditioned on the filtration at time $t-1$, $\F_{t-1}$ is sub-Gaussian random vector, i.e. there exists a parameter $\sigma\geq 0$ such that $\forall \alpha\in\R^d$
\begin{align*}
\E\left[\exp\left(\alpha^\top \wb\nu_t\right)\Big|\F_{t-1}\right]\leq \exp\left(\|\alpha\|_2\sigma^2/2\right)
\end{align*}
\end{assumption}
Asm.~\ref{asm:subgaussian} also implies that $\E\left[\wb\nu_t\Big|\F_{t-1}\right]=0$ which means that after drawing the matrix $\mathbf{\Phi}_t$, the random variable $\wb\nu_t$ is means zero.
A similar assumption on the noise model is assumed in prior analyses of linear bandit \citep{abbasi-yadkori2011improved}.
\begin{lemma}\label{lem:M_t}
Let $\alpha\in\R^d$ be be an arbitrary vector and for any $t\geq0$ define
\begin{align*}
M_t^\alpha :=\exp\left(\sum_i^t\left[\frac{\alpha^\top \mathbf{\Phi}_i^\top\wb\nu_i}{\sigma}-\frac{1}{2}\|\mathbf{\Phi_i}\alpha\|^2_2\right]\right)
\end{align*}
Then, for a stopping time under the filtration $\{\F_t\}_{t=0}^\infty$, $M_\tau^\lambda\leq 1$.
\end{lemma}
\begin{proof}~Lemma.~\ref{lem:M_t}
We first show that $\{M_t^\alpha\}_{t=0}^\infty$ is a supermartingale sequence. Let
\begin{align*}
D_i^\alpha = \exp\left(\frac{\alpha^\top \mathbf{\Phi}_i^\top\wb\nu_i}{\sigma}-\frac{1}{2}\|\mathbf{\Phi_i}\alpha\|^2_2\right)
\end{align*}
Therefore, we can rewrite $\E\left[M^\alpha_t\right]$ as follows:
\begin{align*}
\E\left[M_t^\alpha|\F_{t-1}\right] = \E\left[D_1^\alpha\ldots D_{t-1}^\alpha D_{t}^\alpha|\F_{t-1}\right] = D_1^\alpha\ldots D_{t-1}^\alpha\E\left[ D_{t}^\alpha|\F_{t-1}\right]\leq M_{t-1}^\alpha
\end{align*}
The last inequality follows since $\E\left[ D_{t}^\alpha|\F_{t-1}\right]\leq 1$ due to Assumption~\ref{asm:subgaussian}, therefore since for the first time step $\E\left[M_1^\alpha\right]\leq 1$, then $\E\left[M_t^\alpha\right]\leq 1$. For a stopping time $\tau$, Define a variable $\wo{M}_t^\alpha = M_{\min\{t,\tau\}}^\alpha$ and since $\E\left[M_\tau^\alpha\right]= \E\left[\lim\inf_{t\rightarrow\infty}\wo{M}_t^\alpha\right]\leq \lim\inf_{t\rightarrow \infty}\E\left[\wo{M}_t^\alpha\right]\leq 1$, therefore the Lemma.~\ref{lem:M_t} holds.
\end{proof}

Let's defined the following quantities for self-normalized processes;
\begin{align*}
S_t := \sum_i^t \mathbf{\Phi}_i^\top\wb\nu_i, ~~~~~ \chi_t := \sum_{i=0}^t  \mathbf{\Phi}_i^\top\mathbf{\Phi}_i, ~~~~~ \wo\chi_t = \chi_t+\wt\chi
\end{align*}
where $\wt\chi$ is a ridge regularization matrix and usually is equal to $\lambda I$.
\begin{lemma} \label{lem:self}[Extension to Self-normalized bound in \cite{abbasi-yadkori2011improved}] For a stopping time $\tau$ and filtration $\{\F_t\}_{t=0}^\infty$, with probability at least $1-\delta$
\begin{align*}
\|S_\tau\|_{\wo\chi_\tau^{-1}}\leq 2\sigma^2\log(\frac{\det\left(\wo\chi_t\right)^{1/2}\det(\wt\chi)}{\delta})
\end{align*}
\end{lemma}
\begin{proof}~Lemma.~ \ref{lem:self}
Given the definition of the parameters of self-normalized process, we can rewrite $M_t^\alpha$ as follows;
\begin{align*}
M_t^\alpha = \exp\left(\frac{\alpha^\top S_t}{\sigma}-\frac{1}{2}\|\alpha\|_{\chi_t}\right)
\end{align*}
Consider $\Omega$ as a Gaussian random vector, denoted as $f(\Omega=\alpha)$, with covariance matrix of $\wo \chi^{-1}$. Define $M_t:=\E\left[M_t^\Omega|\F_\infty\right]$, which also results in $\E\left[M_t\right]=\E\left[\E\left[M_t^\Omega|\Omega\right]\right]\leq 1$. Therefore
\begin{align*}
M_t=&\int_{\Re^d}\exp\left(\frac{\alpha^\top S_t}{\sigma}-\frac{1}{2}\|\alpha\|_{\chi_t}\right)f(\alpha)d\alpha\\
%
=&\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\frac{1}{2}\|S_t/\sigma\|^2_{\chi_t^{-1}}\right)f(\alpha)d\alpha\\
%
=&\sqrt{\frac{\det\left(\wt\chi\right)}{\left(2\pi\right)^d}}\exp\left(\frac{1}{2}\|S_t/\sigma\|_{\chi_t^{-1}}\right)\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\frac{1}{2}\|\alpha\|^2_{\wt\chi}\right)d\alpha
\end{align*}
Since $\chi_t$ and $\wt\chi$ are positive semi definite and positive definite respectively, we have 
\begin{align*}
\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\|\alpha\|^2_{\wt\chi}&= \|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}+\|\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}-\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}\\
&=\|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}+\|\S_t/\sigma\|^2_{\chi_t^{-1}}-\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}
\end{align*}
Therefore, 
\begin{align*}
M_t=&\sqrt{\frac{\det\left(\wt\chi\right)}{\left(2\pi\right)^d}}\exp\left(\frac{1}{2}\|S_t/\sigma\|_{\left(\wt\chi+\chi_t\right)^{-1}}\right)\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}\right)d\alpha\\
=&\left(\frac{\det\left(\wt\chi\right)}{\det\left(\wt\chi+\chi_t\right)}\right)^{1/2}\exp\left(\frac{1}{2}\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}\right)
\end{align*}
Since $\E\left[M_\tau\right]\leq 1$ we have
\begin{align*}
\Prob\left(\|S_\tau\|^2_{\left(\wt\chi+\chi_\tau\right)^{-1}}\leq 2\sigma\log\left(\frac{\det\left(\wt\chi+\chi_\tau\right)^{1/2}}{\delta\det\left(\wt\chi\right)^{1/2}}\right)\right)
\leq \frac{\E\left[\exp\left(\frac{1}{2}\|S_\tau/\sigma\|^2_{\left(\wt\chi+\chi_\tau\right)^{-1}}\right)\right]}{\left(\frac{\det\left(\wt\chi+\chi_\tau\right)}{\delta\det\left(\wt\chi\right)}\right)^{1/2}}\leq \delta
\end{align*}
Where the Markov inequality is deployed for the final step. 
The stopping is considered to be the time step as the first time in the sequence when the concentration in the Lemma.~\ref{lem:self} does not hold. 
\end{proof}
\paragraph{Regret Decomposition}
Let's restate the definition of the expected regret and expected Bayesian regret.
\begin{align*}
\textbf{Reg}_T:=\sum_t^T V^{\omega^*}_{\pi^*}- V^{\omega^*}_{\pi_t}
\end{align*}
where $\pi_t$ is the deployed policy at episode $t$ induced by $\omega^t$, $\pi_t(x,a)=a=\arg\max_{a'}\omega_t\phi(x,a')$ and $V^{\omega}_{\pi}$ is the value of policy $\pi$ on model derived by $\omega$\footnote{In general, the analysis also hold for general class of policies (stochastic) as long as the mapping from $\omega$ to policy given and fixed for oracle and the RL algorithm}. The RHS for model based counterpart is  $V^{M^*}_{\pi^*} - V^{M^*}_{\pi_t}$. When there is a prior over the model choice $\omega^*$  the expected Bayesian Regret might be target of study. 
\begin{align*}
\textbf{BayesReg}_T:&=\E_{\omega^*}\left[\textbf{Reg}_T\right]:=\E_{\omega*}\left[\sum_t^T V^{\omega^*}_{\pi^*}(x_t^0)- V^{\omega^*}_{\pi_t}(x_t^0)\right]\\
%
&=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}(x_t^0)- V^{\omega^*}_{\pi_t}(x_t^0)\big|\mathcal{H}_t\right]\right]\\
%
&=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}(x_t^0)- V^{\omega^t}_{\pi_t}(x_t^0)\big|\mathcal{H}_t\right]\right]+\E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\omega_t}_{\pi_t}(x_t^0)- V^{\omega^*}_{\pi_t}(x_t^0)\big|\mathcal{H}_t\right]\right]\\ 
\end{align*}
Here $\mathcal{H}_t$ is a multivariate random sequence which indicates history at the beginning of episode $t$, including $x_t^0$, and  $\omega_t$ is the model parameter chosen through Thompson Sampling. Since the $\omega_t$ and $\omega^*$ are equally distributed conditioned on $\mathbb{H}_t$,  the term $\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}- V^{\omega_t}_{\pi_t}\big|\mathcal{H}_t\right]\right] = 0$ and as a consequence, the first term in the RHS of the last equality is zero. (This term of optimism analysis, when $\omega_t$ is the optimistic choice is zero.)

% Therefore;

% \begin{align*}
% \textbf{BayesReg}_T=\sum_t^T\E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\omega_t}_{\pi_t}- V^{\omega^*}_{\pi_t}\big|\mathcal{H}_t\right]\right]
% \end{align*}
% Which can be interpreted as the deviation of the sampled model and the underlying model under the optimal policy of the sampled model.
For a given state $x_t^0$, the value of the optimal policy $\pi_t$ of model $\omega^t$ under the very same model $\omega^t$  is equal to 

\begin{align*}
V^{\omega_t}_{\pi_t}(x_t^0)=\phi(x_t^0,\pi_t(x_t^0))^\top\omega_t = \E\left[{r}_{\omega_t}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\omega_t}(x'|x_t^0,\pi_t(x_t^0))V^{\omega_t}_{\pi_t}(x')
\end{align*}
and for  $\pi^*$ under  model $\omega^*$  is equal to 
\begin{align*}
V^{\omega^*}_{\pi^*}(x_t^0)=\phi(x_t^0,\pi^*(x_t^0))^\top\omega^* = \E\left[{r}_{\omega^*}(x_t^0,\pi^*(x_t^0))\right]+\int_{x'}T_{\omega^*}(x'|x_t^0,\pi^*(x_t^0))V^{\omega^*}_{\pi^*}(x')
\end{align*}
% \eb{It would be good to use consistent notation here, putting the policy in the superscript and only having the state in the in parentheses. If we want to discuss Q values then we could do $Q^{\pi_t}(x,\pi^*(s))$}.
while $\phi(x_t^0,\pi_t(x_t^0))^\top\omega_t$ is value of $\pi_t$ under model $\omega_t$ at state $x_t^0$ which is also the optimal value at state $x_t^0$ under the model $\omega_t$, $\phi(x_t^0,\pi^*(x_t^0))^\top\omega_t$ is the value of following $\pi^*(x_t^0)$ for one step and then follow $\pi_t$ for the remaining part of horizon. 
% \eb{**I think here we are making a stronger assumption-- that the Q value under other policies is also linear. This assumption should be made in the main text if we need it.}

Furthermore, the value of  $\pi_t$ under  model $\omega^*$  is as follows:

\begin{align*}
V^{\omega^*}_{\pi_t}(x_t^0)&=\E\left[{r}_{\omega^*}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\omega^*}(x'|x_t^0,\pi_t(x_t^0))V^{\omega^*}_{\pi_t}(x')\\
% &=\E\left[{r}_{\omega^*}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\omega^*}(x'|x_t^0,\pi_t(x_t^0))V_{\omega^*}(x',\pi_t)
\end{align*}

Deploying the variable we defined before, we can write the upper bound on the $\textbf{BayesReg}_T$;

\begin{align*}
\textbf{BayesReg}_T\leq\sum_t^T 
\E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[\phi(x_t^0,\pi_t(x_t^0))^\top\omega_t- V^{\omega^*}_{\pi_t}(x_t^0)\big|\mathcal{H}_t\right]\right]
\end{align*}
Since
\begin{align*}
\phi(x_t^0,\pi_t(x_t^0))^\top\omega^*= \E\left[{r}_{\omega^*}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\omega^*}(x'|x_t^0,\pi_t(x_t^0))V_{\omega^*}(x',\pi^*)
\end{align*}
the RHS term can be decomposed as follows;
\begin{align*}
&\phi(x_t^0,\pi_t(x_t^0))^\top\omega_t- V^{\omega^*}_{\pi_t}(x_t^0)=\\
&\quad\quad~\phi(x_t^0,\pi_t(x_t^0))^\top\omega_t-\phi(x_t^0,\pi_t(x_t^0))^\top\omega^*+\phi(x_t^0,\pi_t(x_t^0))^\top\omega^*- V^{\omega^*}_{\pi_t}(x_t^0)\\
&\quad\quad=\phi(x_t^0,\pi_t(x_t^0))^\top\left(\omega_t-\omega^*\right)+\phi(x_t^0,\pi_t(x_t^0))^\top\omega^*- V^{\omega^*}_{\pi_t}(x_t^0)\\
&\quad\quad=\phi(x_t^0,\pi_t(x_t^0))^\top\left(\omega_t-\omega^*\right)+\int_{X^1_t}T_{\omega^*}(X^1_t|x_t^0,\pi_t(x_t^0))\left(\underbrace{V_{\omega^*}(X^1_t,\pi^*)-V_{\omega^*}(X^1_t,\pi_t)}_\text{(a)}\right)
\end{align*}
where $(a)$ can be decomposed the same way as $V_{\omega^*}(x^0_t,\pi^*)-V_{\omega^*}(x^0_t,\pi_t)$. The remaining is to show each of these parts are bounded. 
% \begin{align*}
% (c): V_{\omega^*}(x_t^1,\pi^*)-V_{\omega^*}(x_t^1,\pi_t)=\phi(x_t^1,\pi_t(x_t^1))^\top\omega^*-\phi(x_t^1,\pi_t(x_t^))^\top\omega^*+\phi(x_t^0,\pi_t(x_t^0))^\top\omega^*- V^{\omega^*}_{\pi_t}(x_t^0)\\
% \end{align*}
%
\begin{lemma}[Confidence ellipsoid for problem in Eq.~\ref{eq:Bayesian_model}]\label{lem:conf}
For a matrix problem in Eq.~\ref{eq:Bayesian_model}, given a sequence of $\lbrace\mathbf{\Phi}_i,\mathbf{R}_i\rbrace_{i=1}^{t}$, under the Asm.~\ref{asm:subgaussian} and the following estimator for $\wh\omega_t$
\begin{align*}
\wh\omega_t:= \left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\mathbf{\wb R}_i\right)
\end{align*}
with probability at least $1-\delta$
\begin{align*}
\|\wh\omega_t-\omega^*\|_{\wo\chi_t}\leq \sigma\sqrt{2d\log\left(\frac{1+tL^2/\lambda}{\delta}\right)}+\lambda^{1/2}L_\omega
\end{align*}
where $\|\omega^*\|_2\leq L_\omega$ and $trace{\mathbf{\Phi}(\cdot)\mathbf{\Phi}(\cdot)^\top}\leq L$. 
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:conf}]
Given the estimator $\wh\omega_t$ we have the following:
\begin{align*}
\wh\omega_t&=\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\left(\mathbf{\Phi}_i\omega^* + \wb\nu_i\right)\right)\\
&=\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\wb\nu_i\right)\\
&+ \left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)\omega^*\\
&-\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\omega^*\\
\end{align*}
therefore, for any vector $\zeta\in\Re^d$
\begin{align*}
\zeta^\top\wh\omega_t-\zeta^\top\omega^*&=\zeta^\top\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\wb\nu_i\right)\\
&-\zeta^\top\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\omega^*
\end{align*}
As a results, 
applying Cauchy-Schwarz inequality and inequalities $\|\omega^*\|_{\wo\chi_t^{-1}}\leq \frac{1}{\lambda\left(\wo\chi_t\right)}\|\omega^*\|_2\leq \frac{1}{\lambda}\|\omega^*\|_2$ we get
\begin{align*}
|\zeta^\top\wh\omega_t-\zeta^\top\omega^*|&=\|\zeta\|_{\wo\chi_t^{-1}}\|\sum_i^t\left(\mathbf{\Phi}_i^\top\wb\nu_i\right)\|_{\wo\chi_t^{-1}}-\lambda\|\zeta\|_{\wo\chi_t^{-1}}\|\omega^*\|_{\wo\chi_t^{-1}}\\
&\leq \|\zeta\|_{\wo\chi_t^{-1}}\|\left(\|\sum_i^t\left(\mathbf{\Phi}_i^\top\wb\nu_i\right)\|_{\wo\chi_t^{-1}}+\lambda^{1/2}\|\omega^*\|_2\right)
\end{align*}
where applying self normalized Lemma \ref{lem:self}, with probability at least $1-\delta$
\begin{align*}
|\zeta^\top\wh\omega_t-\zeta^\top\omega^*|\leq \|\zeta\|_{\wo\chi_t^{-1}}\left(2\sigma\log\left(\frac{\det\left(\wo\chi_t\right)^{1/2}}{\delta\det\left(\wt\chi\right)^{1/2}}\right)+\lambda^{1/2}L_\omega\right)
\end{align*}
hold for any $\zeta$. By plugging in $\zeta=\wo\chi_t\left(\wh\omega_t-\omega^*\right)$ %we get the statement in the Lemma \ref{lem:conf}.
we get the following;
\begin{align*}
\|\wh\omega_t-\omega^*\|_{\wo\chi_t}\leq\theta_t(\delta):= \sigma\sqrt{2\log\left(\frac{\det(\wo\chi_t)^{1/2}\det(\lambda I)^{1/2}}{\delta}\right)}+\lambda^{1/2}L_\omega
\end{align*}
The $\det(\wo\chi_t)$ can be written as $\det(\wo\chi_t)=\prod_j^d\alpha_j$ therefore, $trace(\wo\chi_t)=\sum_j^d\alpha_j$. We also know that;
\begin{align*}
    (\prod_j^d\alpha_j)^{1/d}\leq \frac{\sum_j^d\alpha_j}{d}
\end{align*}
A matrix extension to Lemma 10 and 11 in \cite{abbasi-yadkori2011improved} results in  $\det(\wo\chi_t)\leq \left(\frac{trace(\wo\chi_t)}{d}\right)^d$ while we have $trace(\wo\chi_t)=trace(\lambda I)+\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i\leq d\lambda+tL$, therefore the main statement of Lemma \ref{lem:conf} goes through.
\end{proof}



% \eb{Wait, I'm confused. I thought we just proved Lemma 3. And the below is not stated as a lemma. Could you clarify please?}

% \begin{lemma}[Determinant inequality]
% For a matrix problem in Eq.~\ref{eq:Bayesian_model}, given a sequence of $\lbrace\mathbf{\Phi}_i,\mathbf{R}_i\rbrace_{i=1}^{t}$, and under $trace{\mathbf{\Phi}(\cdot)\mathbf{\Phi}(\cdot)^\top}\leq L$  we have:
% \begin{align*}
% \det\left(\wo\chi_t\right)\leq (\lambda+tL^2/d)^d\quad,\quad \sum
% \end{align*}
% \end{lemma}

For the regret, condition on $\mathcal{H}_t$, then drawn $\mathbf{\Phi}_t$ following $\pi_t$
\begin{align*}
&\phi(x_t^0,\pi_t(x_t^0))^\top\omega_t- V^{\omega^*}_{\pi_t}(x_t^0)\\
&\quad\quad\quad\quad=\mathbbm{1}^\top\mathbf{\Phi}_t\left(\omega_t-\omega^*\right)=\mathbbm{1}^\top\mathbf{\Phi}_t\wo\chi_t^{-1/2}\wo\chi_t^{1/2}\left(\omega_t-\omega^*\right)\leq \sqrt{H} \|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\|\omega_t-\omega^*\|_{\wo\chi_t}
\end{align*}
Therefore, by running the \TS, we get a distribution over the whole history and for a given history we have;
\begin{align*}
\textbf{BayesReg}_T&\leq\sqrt{H}
\E\left[\sum_t^T \|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\|\omega_t-\omega^*\|_{\wo\chi_t}\right]\\
&\leq \sqrt{H}
\E\left[\sum_t^T \|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\|\omega_t-\wh\omega\|_{\wo\chi_t}+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\|\omega^*-\wh\omega\|_{\wo\chi_t}\right]\\
&\leq 2\sqrt{H}
\E\left[\sum_t^T\theta_t(\delta)\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right]
\end{align*}
Since we know assumed the maximum cumulative return of each episode is as most $1$, we have;
\begin{align*}
\textbf{BayesReg}_T\leq 2\sqrt{H}
\E\left[\sum_t^T\min\lbrace\theta_t(\delta)\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}},1\rbrace\right]\leq 2\sqrt{H}
\E\left[\sum_t^T\theta_t(\delta)\min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}},1\rbrace\right]
\end{align*}
Moreover, at time $T$, we can use Jensen's inequality, exploit the fact that $\theta_t(\delta)$ is an increasing function of $t$ and have
\begin{align}\label{eq:BR1}
\textbf{BayesReg}_T&\leq 2\sqrt{H}
\E\left[\sqrt{T\theta_T(\delta)^2\sum_t^T\min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}},1\rbrace}\right]\nonumber\\
&\leq 2\sqrt{H}
\left(\sigma\sqrt{2\log\left(\frac{1+tL^2/\lambda}{\delta}\right)}+\lambda^{1/2}L_\omega\right)\E\left[\sqrt{T\sum_t^T\min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}},1\rbrace}\right]
\end{align}
Using the fact that for any scalar $\alpha$ such that $0\leq \alpha\leq 1$, then $\alpha\leq 2\log(1+\alpha)$, we can rewrite the latter part of Eq.~\ref{eq:BR1}
\begin{align*}
\sqrt{\sum_t^T\min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}},1\rbrace}\leq 2\sum_t^T\log\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)
\end{align*}
In order to bound the RHS of the this inequality, we use generalized matrix determinant lemma.
\begin{align*}
\det\left(\wo\chi_T\right)&=\det\left(\wo\chi_{T-1}+\mathbf{\Phi}_T^\top\mathbf{\Phi}_T\right)\\
&=\det\left(I_H+\mathbf{\Phi}_T\wo\chi_t^{-1}\mathbf{\Phi}_T^\top\right)\det\left(\wo\chi_{T-1}\right)\\
&=\prod_t^T\det\left(I_H+\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top\right)\det\left(\wt\chi\right)
\end{align*}
From linear algebra, and given a time step $t$, we know the characteristic polynomial of the matrix $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ is $CP_t(\wb\lambda)=\det(\wb\lambda I_H-\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top)$. If the set $\lbrace\lambda_1,\lambda_2,\ldots,\lambda_d\rbrace$ represent the eigenvalues of $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ where $\lambda_i\geq\lambda_j$ if $i\geq j$, one can rewrite $CP_t(\wb\lambda)$ as follows;
\begin{align*}
    CP(\wb\lambda) = (\wb\lambda-\lambda_1)(\wb\lambda-\lambda_2)\cdots (\wb\lambda-\lambda_H)
\end{align*} 
by adding the matrix $I_H$ to $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ where $\lambda_i\geq\lambda)j$, we get $CP_t'(\wb\lambda)=\det(\wb\lambda I_H-I_H-\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top)$, therefore;
\begin{align*}
    CP_t'(\wb\lambda) = (\wb\lambda-1-\lambda_1)(\wb\lambda-1-\lambda_2)\cdots (\wb\lambda-1-\lambda_H)
\end{align*} 
and the eigenvalues of $I_H+\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ are shifted eigenvalues of $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ by $+1$, i.e. $\lbrace\lambda_1+1,\lambda_2+1,\ldots,\lambda_d+1\rbrace$. Since $\xi^\top\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top\xi=\left(\mathbf{\Phi}{\wo\chi_t^{-1/2}}^\top\xi\right)^\top\left(\mathbf{\Phi}{\wo\chi_t^{-1/2}}^\top\xi\right)$ all the eigenvalues $\lbrace\lambda_1,\lambda_2,\ldots,\lambda_d\rbrace$ are non-negative. As a results,
\begin{align*}
    \det\left(I_H+\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top\right)\geq \left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)
\end{align*}
As a consequence; 
\begin{align*}
    \det\left(\wo\chi_T\right)\geq\det\left(\wt\chi\right) \prod_t^T\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)
\end{align*}
Therefore,
\begin{align}\label{eq:xx}
2\sum_t^T\log\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)\leq 2\left(\log\left(\det\left(\wo\chi_T\right)\right)-\log\left(\det\left(\wt\chi\right)\right)\right)\leq 2 d\log(\lambda + TL^2/d)
\end{align}
Substituting the RHS of Eq.~\ref{eq:xx} into Eq.~\ref{eq:BR1}, we get 
\begin{align*}
\textbf{BayesReg}_T
&\leq 2\sqrt{H}
\left(\sigma\sqrt{2d\log\left(\frac{1+TL^2/\lambda}{\delta}\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2T d\log(\lambda + TL^2/d)}
\end{align*}
which is the the statement in the Theorem.

% \paragraph{Conjecture on optimism}: In the previous proof, we used the fact that $\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}- V^{\omega_t}_{\pi_t}\big|\mathcal{H}_t\right]\right] = 0$. This is true since the prior and likelihood are known to the agent. Consider the case where the agent does not have access to prior and posterior. In this case, the agent, at time $t$, fits a multi-variate Gaussian around $\wh\omega_t$ with the covariance induced by Eq.~\ref{eq:beta-beta*} multiplied by $\sqrt{d}$ and use it to draw $\omega_t$. Then applying a similar arguemnt as \citet{abeille2017linear}, we might be able to show that $\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}- V^{\omega_t}_{\pi_t}\big|\mathcal{H}_t\right]\right] \leq$. Therfore, for both Bayesian regret bound Frequentist bound for Thompson Sampling without knowing the prior and likelihod we get a regret bound of $\widetilde\mathcal{O}(d^{1.5}\sqrt{HT})$.


==> Sections/old-10-Theory-old.tex <==
\section{Bayesian Regret}
Let's consider the following linear model over the $Q$ functions and returns for episodic with episode length of $H$. (We consider the discount factor to be any number $0\leq \gamma\leq 1$)



\begin{equation}\label{eq:Bayesian_model}
\Psi\mathbf{R} = \mathbf{\Phi}(x^{\{1:H\}},a^{\{1:H\}})\beta +\Psi \nu(x^{\{1:H\}},a^{\{1:H\}})~,~~ \textit{where}~,~\Psi:=\left[
  \begin{tabular}{ccccc}
  1 & $\gamma$ & $\gamma^2$ &$\ldots$ & $\gamma^{H-1}$\\
  0 & 1 & $\gamma$ &  $\ldots$ & $\gamma^{H-2}$\\
  0 & 0 & $1$ & $\ldots$ &$\vdots$ \\
  $\vdots$ & $\ldots$ & $\ldots$& $\ldots$ & $\vdots$\\
  $0$ & $\ldots$ & $\ldots$& $\ldots$ & 1
  \end{tabular}
\right]
\end{equation}
Where the Q function is a linear function of $\phi(x,a)\in \R^d$, which is $Q(x,a):=\phi(x,a)\beta$. For the theoretical analysis we consider the feature representation also contains features of action. The vector $\mathbf{R}\in \Re^H$ is the random vector of rewards in a episode. The matrix $\mathbf{\Phi}(x^{\{1:H\}},a^{\{1:H\}})\in\Re^{H\times d}$ is row-wised concatenation of sequence of state-action features, $\phi(x,a)$ under a given policy, also any instance of $\|\mathbf{\Phi}(x^{\{1:H\}},a^{\{1:H\}})\|_2\leq L$. The vector $\nu(x^{\{1:H\}},a^{\{1:H\}})\in\Re^H$% \sim \N(0,\Sigma_\epsilon(x_{\{1:H\}},a_{\{1:H\}))$
is a state-action dependent noise vector where, for any $h'$, the noises after time step $h'$, $\nu^{h=i\geq h'}$, are independent from the noises before time step $h'$, $\nu^{h=i< h'}$ condition on $(x^h,a^h)$, the state action pair at time step $h$. Moreover, since the underlying model of environment is assumed to be MDP, the noise at time step $h$, $\nu^h$ models the induces noise by stochasticity of transition distribution to state $x^h$, i.e. $f(x^h|x^{h-1},a^{h-1})$, and the stochasticity of reward at time step $h$, i.e. $r(x^h,a^h)$.
In the Bayesian approach, we consider a Gaussian prior over the parameter vector $\beta\sim\N(0,\sigma I)$, then exploit the samples to compute the posterior. After computing the posterior, we deploy \TS and draw a vector $\beta$, then follow the policy induced by $\beta$. We then collect the generated sample to update the posterior and the policy for next episode. 

In the following, we show after $T$ episodes of following \TS, the estimated $\hat{b}$ concentrates. The main body of the following analyses on concentration of measure is a matrix extension to contextual linear bandit analyses \cite{abbasi-yadkori2011improved,chu2011contextual,li2010contextual,rusmevichientong2010linearly,dani2008stochastic} and self normalized processes\citep{de2004self}. For the regret analysis, we extend the analysis in frequentest and Bayesian regret literature \cite{osband2014generalization,osband2013more,jaksch2010near}

In order to ease the analysis, we exploit the property of the matrix $\Psi$ where
\begin{align*}
\Psi^{-1}=\left[
  \begin{tabular}{ccccc}
  1 & $-\gamma$ & 0 &$\ldots$ & 0\\
  0 & 1 & -$\gamma$ &  $\ldots$ & 0\\
  0 & 0 & $1$ & $\ldots$ &$\vdots$ \\
  $\vdots$ & $\ldots$ & $\ldots$& $\ldots$ & $\vdots$\\
  $0$ & $\ldots$ & $\ldots$& $\ldots$ & 1
  \end{tabular}
\right]
\end{align*}
therefore, the Eq.~\ref{eq:Bayesian_model} can be written as follows:

\begin{equation}
\mathbf{R} = \Psi^{-1}\mathbf{\Phi}(x^{\{1:H\}},a^{\{1:H\}})\beta + \nu(x^{\{1:H\}},a^{\{1:H\}})
\end{equation}

\begin{assumption}[Sub-Gaussian random vector \citep{hsu2012tail}]\label{asm:subgaussian}
The noise model at time $t$, condition on the filtration at time $t-1$, $\F_{t-1}$ is sub-Gaussian random vector, i.e. there exists a parameter $\sigma\geq 0$ such that $\forall \alpha\in\R^d$
\begin{align*}
\E\left[\exp\left(\alpha^\top\mathbf{\Phi}_t^\top\Psi' \nu_t\right)\Big|\F_{t-1}\right]\leq \exp\left(\|\alpha\|_{\Psi^{-1}\mathbf{\Phi}_t}^2\sigma^2/2\right)
\end{align*}
where $\Psi':={\Psi^{-1}}^\top$
\end{assumption}
The Asm.~\ref{asm:subgaussian} also interprets that $\E\left[\mathbf{\Phi}_t^\top\Psi' \nu_t\Big|\F_{t-1}\right]=0$ which is a common assumption for regression and linear bandits analysis. For the MDP case, this assumption is satisfied when $\E\left[\nu_i\Big|\F_{t-1},x^{\{1:i\}},a^{\{1:i\}}\right]=0$, in other words, $\E\left[\mathbf{\Phi}_t^\top\Psi' \nu_t\Big|\F_{t-1}\right]$ can be written as;
\begin{align*}
\begin{split}
\E\left[\E\left[\ldots\E\left[\E\left[\left[\nu^{1}\left(\phi^{1}-\gamma\phi^{2}\right)+\ldots+\nu^{H-1}\left(\phi^{H-1}-\gamma\phi^{H}\right)+\right.\right.\right.\right.\right.\\
\left.\left.\left.\left.\left.\nu^{H}\left(\phi^{H}\right)|x^{H},a^{H}\right]|x^{H-1},a^{H-1}\right]\ldots|x^{1},a^{1}\right]\right]\Big|\F_{t-1}\right]
\end{split}
\end{align*}
which is zero if $\E\left[\nu^{i}\left(\phi^{i}-\gamma\phi^{i+1}\right)\Big|x^{i},\F_{t-1}\right]=0$. This is a reasonable assumption for MDPs since $\nu_i$ carries the noise on transition to $x_i$ and the reward after taking action $a_i$ while does not carry the noise model of transition to the next state. In other word, $\nu_i$ models the stochasticity of $f(x^{i}|x^{i-1},a^{i-1})$ and $r(x^{i},a^{i})$.


\begin{lemma}\label{lem:M_t}
Let $\alpha\in\R^d$ be arbitrary and for any $t\geq0$ define
\begin{align*}
M_t^\alpha :=\exp\left(\sum_i^t\left[\frac{\alpha^\top \mathbf{\Phi}_i^\top\Psi'\nu_i}{\sigma}-\frac{1}{2}\|\alpha^\top \mathbf{\Phi_i}^\top\Psi'\|^2_2\right]\right)
\end{align*}
For a stopping time (specified mathematically latter) under the filtration $\{\F_t\}_{t=0}^\infty$, $M_\tau^\lambda\leq 1$.
\end{lemma}
\begin{proof}~Lemma.~\ref{lem:M_t}
We first show that $\{M_t^\alpha\}_{t=0}^\infty$ is supermartingale sequence. Let
\begin{align*}
D_i^\alpha = \exp\left(\frac{\alpha^\top \mathbf{\Phi}_i^\top\Psi'\nu_i}{\sigma}-\frac{1}{2}\|\alpha^\top \mathbf{\Phi_i}^\top\Psi'\|^2_2\right)
\end{align*}
Therefore, we can rewrite $\E\left[M^\alpha_t\right]$ as follows:
\begin{align*}
\E\left[M_t^\alpha|\F_{t-1}\right] = \E\left[D_1^\alpha\ldots D_{t-1}^\alpha D_{t}^\alpha|\F_{t-1}\right] = D_1^\alpha\ldots D_{t-1}^\alpha\E\left[ D_{t}^\alpha|\F_{t-1}\right]\leq M_{t-1}^\alpha
\end{align*}
The last inequality follows since $\E\left[ D_{t}^\alpha|\F_{t-1}\right]\leq 1$ due the Asm.~\ref{asm:subgaussian}, therefore, $\E\left[M_t^\alpha\right]\leq 1$. For a stopping time $\tau$, lets define a variable $\wo{M}_t^\alpha = M_{\min\{t,\tau\}}^\alpha$ and since $\E\left[M_\tau^\alpha\right]= \E\left[\lim\inf_{t\rightarrow\infty}\wo{M}_t^\alpha\right]\leq \lim\inf_{t\rightarrow \infty}\E\left[\wo{M}_t^\alpha\right]\leq 1$, therefore the Lemma.~\ref{lem:M_t} holds.
\end{proof}

Let's defined the following quantities for self-normalized processes;
\begin{align*}
S_t := \sum_i^t \mathbf{\Phi}_i^\top\Psi'\nu_i, ~~~~~ \chi_t := \sum_{i=0}^t  \mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i, ~~~~~ \wo\chi_t = \chi_t+\wt\chi
\end{align*}
where $\wt\chi$ is a ridge regularization matrix and usually is equal to $\lambda I$.
\begin{lemma} \label{lem:self}[Extension to Self-normalized bound in \cite{abbasi-yadkori2011improved}] For a stopping time $\tau$ and filtration $\{\F_t\}_{t=0}^\infty$, with probability at least $1-\delta$
\begin{align*}
\|S_\tau\|_{\wo\chi_\tau^{-1}}\leq 2\sigma^2\log(\frac{\det\left(\wo\chi_t\right)^{1/2}\det(\wt\chi)}{\delta})
\end{align*}
\end{lemma}
\begin{proof}~Lemma.~ \ref{lem:self}
Given the definition of the parameters of self-normalized process, we can rewrite $M_t^\alpha$ as follows;
\begin{align*}
M_t^\alpha = \exp\left(\frac{\alpha^\top S_t}{\sigma}-\frac{1}{2}\|\alpha\|_{\chi_t}\right)
\end{align*}
Consider $\Omega$ as a Gaussian random vector, denoted as $f(\Omega=\alpha)$, with covariance matrix of $\wo \chi^{-1}$. Define $M_t:=\E\left[M_t^\Omega|\F_\infty\right]$, which also results in $\E\left[M_t\right]=\E\left[\E\left[M_t^\Omega|\Omega\right]\right]\leq 1$. Therefore
\begin{align*}
M_t=&\int_{\Re^d}\exp\left(\frac{\alpha^\top S_t}{\sigma}-\frac{1}{2}\|\alpha\|_{\chi_t}\right)f(\alpha)d\alpha\\
%
=&\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\frac{1}{2}\|S_t/\sigma\|^2_{\chi_t^{-1}}\right)f(\alpha)d\alpha\\
%
=&\sqrt{\frac{\det\left(\wt\chi\right)}{\left(2\pi\right)^d}}\exp\left(\frac{1}{2}\|S_t/\sigma\|_{\chi_t^{-1}}\right)\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\frac{1}{2}\|\alpha\|^2_{\wt\chi}\right)d\alpha
\end{align*}
Since $\chi_t$ and $\wt\chi$ are positive semi definite and positive definite respectively, we have 
\begin{align*}
\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\|\alpha\|^2_{\wt\chi}&= \|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}+\|\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}-\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}\\
&=\|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}+\|\S_t/\sigma\|^2_{chi_t^{-1}}-\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}
\end{align*}
Therefore, 
\begin{align*}
M_t=&\sqrt{\frac{\det\left(\wt\chi\right)}{\left(2\pi\right)^d}}\exp\left(\frac{1}{2}\|S_t/\sigma\|_{\left(\wt\chi+\chi_t\right)^{-1}}\right)\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}\right)d\alpha\\
=&\left(\frac{\det\left(\wt\chi\right)}{\det\left(\wt\chi+\chi_t\right)}\right)^{1/2}\exp\left(\frac{1}{2}\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}\right)
\end{align*}
Since $\E\left[M_\tau\right]\leq 1$ we have
\begin{align*}
\Prob\left(\|S_\tau\|^2_{\left(\wt\chi+\chi_\tau\right)^{-1}}\leq 2\sigma\log\left(\frac{\det\left(\wt\chi+\chi_\tau\right)^{1/2}}{\delta\det\left(\wt\chi\right)^{1/2}}\right)\right)
\leq \frac{\E\left[\exp\left(\frac{1}{2}\|S_\tau/\sigma\|^2_{\left(\wt\chi+\chi_\tau\right)^{-1}}\right)\right]}{\left(\frac{\det\left(\wt\chi+\chi_\tau\right)}{\delta\det\left(\wt\chi\right)}\right)^{1/2}}\leq \delta
\end{align*}
Where the Markov inequality is deployed for the final step. 
The stopping is considered to be the time step as the first time in the sequence when the concentration in the Lemma.~\ref{lem:self} does not hold. 
\end{proof}
\paragraph{Regret Decomposition}
Let's restate the definition of the expected regret and expected Bayesian regret.
\begin{align*}
\textbf{Reg}_T:=\sum_t^T V^{\beta^*}_{\pi^*}- V^{\beta^*}_{\pi_t}
\end{align*}
where $\pi_t$ is the deployed policy at episode $t$ induced by $\beta^t$, $\pi_t(x,a)=a=\arg\max_{a'}\beta_t\phi(x,a')$ and $V^{\beta}_{\pi}$ is the value of policy $\pi$ on model derived by $\beta$\footnote{In general, the analysis also hold for general class of policies (stochastic) as long as the mapping from $\beta$ to policy given and fixed for oracle and the RL algorithm}. The RHS for model based counterpart is  $V^{M^*}_{\pi^*} - V^{M^*}_{\pi_t}$. When there is a prior over the model choice $\beta^*$  the expected Bayesian Regret might be target of study. 
\begin{align*}
\textbf{BayesReg}_T:&=\E_{\beta^*}\left[\textbf{Reg}_T\right]:=\E_{\beta*}\left[\sum_t^T V^{\beta^*}_{\pi^*}(x_t^0)- V^{\beta^*}_{\pi_t}(x_t^0)\right]
%
=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\beta^*}\left[V^{\beta^*}_{\pi^*}(x_t^0)- V^{\beta^*}_{\pi_t}(x_t^0)\big|\mathcal{H}_t\right]\right]\\
%
&=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\beta^*}\left[V^{\beta^*}_{\pi^*}(x_t^0)- V^{\beta^t}_{\pi_t}(x_t^0)\big|\mathcal{H}_t\right]\right]+\E_{\mathcal{H}_t}\left[\E_{\beta^*}\left[V^{\beta_t}_{\pi_t}(x_t^0)- V^{\beta^*}_{\pi_t}(x_t^0)\big|\mathcal{H}_t\right]\right]\\ 
\end{align*}
Here $\mathcal{H}_t$ is a multivariate random sequence which indicates history at the beginning of episode $t$, including $x_t^0$, and  $\beta_t$ is the model parameter chosen through Thompson Sampling. Since the $\beta_t$ and $\beta^*$ are equally distributed conditioned on $\mathbb{H}_t$,  the term $\left[\E_{\beta^*}\left[V^{\beta^*}_{\pi^*}- V^{\beta_t}_{\pi_t}\big|\mathcal{H}_t\right]\right] = 0$ and as a consequence, the first term in the RHS of the last equality is zero. (This term of optimism analysis, when $\beta_t$ is the optimistic choice is zero.)

% Therefore;

% \begin{align*}
% \textbf{BayesReg}_T=\sum_t^T\E_{\mathcal{H}_t}\left[\E_{\beta^*}\left[V^{\beta_t}_{\pi_t}- V^{\beta^*}_{\pi_t}\big|\mathcal{H}_t\right]\right]
% \end{align*}
% Which can be interpreted as the deviation of the sampled model and the underlying model under the optimal policy of the sampled model.
For a given state $x_t^0$, the value of the optimal policy $\pi_t$ of model $\beta^t$ under the very same model $\beta^t$  is equal to 

\begin{align*}
V_{\beta_t}(x_t^0,\pi_t)=\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t = \E\left[{r}_{\beta_t}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\beta_t}(x'|x_t^0,\pi_t(x_t^0))V_{\beta_t}(x',\pi_t)
\end{align*}
and for  $\pi^*$ under  model $\beta^*$  is equal to 
\begin{align*}
V_{\beta^*}(x_t^0,\pi^*)=\phi(x_t^0,\pi^*(x_t^0))^\top\beta^* = \E\left[{r}_{\beta^*}(x_t^0,\pi^*(x_t^0))\right]+\int_{x'}T_{\beta^*}(x'|x_t^0,\pi^*(x_t^0))V_{\beta^*}(x',\pi^*)
\end{align*}
while $\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t$ is value of $\pi_t$ under model $\beta_t$ at state $x_t^0$ which is also the optimal value at state $x_t^0$ under the model $\beta_t$, $\phi(x_t^0,\pi^*(x_t^0))^\top\beta_t$ is the value of following $\pi^*(x_t^0)$ for one step and then follow $\pi_t$ for the remaining part of horizon. Furthermore, the value of  $\pi_t$ under  model $\beta^*$  is as follows:

\begin{align*}
V_{\beta^*}(x_t^0,\pi_t)&=\E\left[{r}_{\beta^*}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\beta^*}(x'|x_t^0,\pi_t(x_t^0))V_{\beta^*}(x',\pi_t)\\
&=\E\left[{r}_{\beta^*}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\beta^*}(x'|x_t^0,\pi_t(x_t^0))V_{\beta^*}(x',\pi_t)
\end{align*}

Therefore, we can write the upper bound on the $\textbf{BayesReg}_T$;

\begin{align*}
\textbf{BayesReg}_T\leq\sum_t^T 
\E_{\mathcal{H}_t}\left[\E_{\beta^*}\left[\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t- V^{\beta^*}_{\pi_t}(x_t^0)\big|\mathcal{H}_t\right]\right]
\end{align*}
Since
\begin{align*}
\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*= \E\left[{r}_{\beta^*}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\beta^*}(x'|x_t^0,\pi_t(x_t^0))V_{\beta^*}(x',\pi^*)
\end{align*}
the RHS term can be decomposed as follows;
\begin{align*}
&\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t- V^{\beta^*}_{\pi_t}(x_t^0)=\\
&\quad\quad~\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t-\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*+\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*- V^{\beta^*}_{\pi_t}(x_t^0)\\
&\quad\quad=\phi(x_t^0,\pi_t(x_t^0))^\top\left(\beta_t-\beta^*\right)+\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*- V^{\beta^*}_{\pi_t}(x_t^0)\\
&\quad\quad=\phi(x_t^0,\pi_t(x_t^0))^\top\left(\beta_t-\beta^*\right)+\int_{X^1_t}T_{\beta^*}(X^1_t|x_t^0,\pi_t(x_t^0))\left(\underbrace{V_{\beta^*}(X^1_t,\pi^*)-V_{\beta^*}(X^1_t,\pi_t)}_\text{(a)}\right)
\end{align*}
where $(a)$ can be decomposed the same way as $V_{\beta^*}(x^0_t,\pi^*)-V_{\beta^*}(x^0_t,\pi_t)$. The remaining is to show each of these parts are bounded.
% \begin{align*}
% (c): V_{\beta^*}(x_t^1,\pi^*)-V_{\beta^*}(x_t^1,\pi_t)=\phi(x_t^1,\pi_t(x_t^1))^\top\beta^*-\phi(x_t^1,\pi_t(x_t^))^\top\beta^*+\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*- V^{\beta^*}_{\pi_t}(x_t^0)\\
% \end{align*}
%
\begin{lemma}[Confidence ellipsoid for problem in Eq.~\ref{eq:Bayesian_model}]\label{lem:conf}
For a matrix problem in Eq.~\ref{eq:Bayesian_model}, given a sequence of $\lbrace\mathbf{\Phi}_i,\mathbf{R}_i\rbrace_{i=1}^{t}$, under the Asm.~\ref{asm:subgaussian} and the following estimator for $\wh\beta_t$
\begin{align*}
\wh\beta_t:= \left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\mathbf{R}_i\right)
\end{align*}
with probability at least $1-\delta$
\begin{align*}
\|\wh\beta_t-\beta^*\|_{\wo\chi_t}\leq \sigma\sqrt{2\log\left(\frac{1+tL^2/\lambda}{\delta}\right)}+\lambda^{1/2}L_\beta
\end{align*}
where $\|\beta^*\|_2\leq L_\beta$ and $\|\Psi^{-1}\mathbf{\Phi}(\cdot)\|_2\leq L$. 
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:conf}]
Given the estimator $\wh\beta_t$ we have the following:
\begin{align*}
\wh\beta_t&=\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i\beta^* + \nu_i\right)\\
&=\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\\
&+ \left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)\beta^*\\
&-\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\beta^*\\
\end{align*}
therefore, for any vector $\zeta\in\Re^d$
\begin{align*}
\zeta^\top\wh\beta_t-\zeta^\top\beta^*&=\zeta^\top\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\\
&-\zeta^\top\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\beta^*
\end{align*}
As a results, applying Cauchy–Schwarz inequality and inequalities $\|\beta^*\|_{\wo\chi_t^{-1}}\leq \frac{1}{\lambda\left(\wo\chi_t\right)}\|\beta^*\|_2\leq \frac{1}{\lambda}\|\beta^*\|_2$ we get
\begin{align*}
|\zeta^\top\wh\beta_t-\zeta^\top\beta^*|&=\|\zeta\|_{\wo\chi_t^{-1}}\|\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\|_{\wo\chi_t^{-1}}-\lambda\|\zeta\|_{\wo\chi_t^{-1}}\|\beta^*\|_{\wo\chi_t^{-1}}\\
&\leq \|\zeta\|_{\wo\chi_t^{-1}}\|\left(\|\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\|_{\wo\chi_t^{-1}}+\lambda^{1/2}\|\beta^*\|_2\right)
\end{align*}
where applying self normalized Lemma \ref{lem:self}, with probability at least $1-\delta$
\begin{align*}
|\zeta^\top\wh\beta_t-\zeta^\top\beta^*|\leq \|\zeta\|_{\wo\chi_t^{-1}}\left(2\sigma\log\left(\frac{\det\left(\wo\chi_t\right)^{1/2}}{\delta\det\left(\wt\chi\right)^{1/2}}\right)+\lambda^{1/2}L_\beta\right)
\end{align*}
hold for any $\zeta$. By plugging in $\zeta=\wo\chi_t\left(\wh\beta_t-\beta^*\right)$ %we get the statement in the Lemma \ref{lem:conf}.
we get the following;
\begin{align*}
\|\wh\beta_t-\beta^*\|_{\wo\chi_t}\leq \sigma\sqrt{2\log\left(\frac{\det(\wo\chi_t)^{1/2}\det(\lambda I)^{1/2}}{\delta}\right)}+\lambda^{1/2}L_\beta
\end{align*}
The $\det(\wo\chi_t)$ can be written as $\det(\wo\chi_t)=\Pi_j^d\alpha_j$ therefore, $trace(\wo\chi_t)=\sum_j^d\alpha_j$. We also know that;
\begin{align*}
    (\Pi_j^d\alpha_j)^{1/d}\leq \frac{\sum_j^d\alpha_j}{d}
\end{align*}
Therefore, $\det(\wo\chi_t)\leq \left(\frac{trace(\wo\chi_t)}{d}\right)^d$ while we have $trace(\wo\chi_t)=trace(\lambda I)+\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i\leq d\lambda+tL$, the main statement of Lemma \ref{lem:conf} goes through.
\end{proof}




In order to prove Lemma~\ref{lem:conf}, we need the following Lemma which is a direct extension to the Lemma 10 and 11 in \cite{abbasi-yadkori2011improved}.
\begin{lemma}[Determinant inequality]
For a matrix problem in Eq.~\ref{eq:Bayesian_model}, given a sequence of $\lbrace\mathbf{\Phi}_i,\mathbf{R}_i\rbrace_{i=1}^{t}$, and under $\|\mathbf{\Phi}(\cdot)\|_2\leq L$  we have:
\begin{align*}
\det\left(\wo\chi_t\right)\leq (\lambda+tL^2/d)^d\quad,\quad \sum
\end{align*}
\end{lemma}

For the regret, condition on $\mathcal{H}_t$, then drawn $\mathbf{\Phi}_t$ following $\pi_t$
\begin{align*}
&\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t- V^{\beta^*}_{\pi_t}(x_t^0)\\
&\quad\quad\quad\quad=\mathbbm{1}^\top\mathbf{\Phi}_t\left(\beta_t-\beta^*\right)=\mathbbm{1}^\top\mathbf{\Phi}_t\wo\chi_t^{-1/2}\wo\chi_t^{1/2}\left(\beta_t-\beta^*\right)\leq \sqrt{H} \|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\|\beta_t-\beta^*\|_{\wo\chi_t}
\end{align*}
Therefore, by running the \TS, we get a distribution over the whole history and for a given history we have;
\begin{align*}
\textbf{BayesReg}_T\leq\sum_t^T \sqrt{H}
\E\left[\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\|\beta_t-\beta^*\|_{\wo\chi_t}\right]
\end{align*}



==> Sections/old-11-Bayesian.tex <==
\subsection{Bayesian Regret}\label{sec:proof}
The analysis developed in the previous section, up to some minor modification, e.g., change of strategy to \PSRL,  directly applies to Bayesian regret bound, with a furthur union bound over models.

When there is a prior over the $\omega^*$  the expected Bayesian Regret might be target of study. 
\begin{align*}
\textbf{BayesReg}_T:&=\E_{\omega^*}\left[\textbf{Reg}_T\right]:=\E_{\omega*}\left[\sum_t^T V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(X_t^1)\right]\\
%
&=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(X_t^1)\big|\mathcal{H}_t\right]\right]\\
%
\end{align*}
Here $\mathcal{H}_t$ is a multivariate random sequence which indicates history at the beginning of episode $t$, including $X_t^1$ and  $\omega_t$ is the model parameter chosen through \PSRL. 

Condition on the history $\mathcal{H}_t$, we estimate the $\wh \omega_t$ as follows; 
\begin{align*}
\wh\omega_t:= \left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\mathbf{\wb R}_i\right)
\end{align*}
Lemma~\ref{lem:conf} states that with probability at least $1-\delta$, 
$\|\wh\omega_t-\omega^*\|_{\wo\chi_t}\leq\theta_t(\delta)$, $\forall t\leq \tau$. Let construct the confidence interval as follows;
The confidence set $\C_t(\delta)$, condition on $\mathcal{H}_t$ is deterministic. Following \PSRL Alg.~\ref{alg:psrl}, we set $\pi_t$ drawn from the posterior distribution.

Conditioned on $\mathcal{H}_t$, the $\omega_t$ and $\omega^*$ are equally distributed, then we have
\begin{align*}
 \E_{\omega_*}\left[V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)\big|\mathcal{H}_t\right]=\E_{\omega_*}\left[ V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)\big|\mathcal{H}_t\right]   
\end{align*}
therefore, resulting in
\begin{align*}
\textbf{BayesReg}_T:&=\E_{\omega^*}\left[\textbf{Reg}_T\right]:=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(x_t^1)\big|\mathcal{H}_t\right]\right]\\
%
&=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)+V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(X_t^1)\big|\mathcal{H}_t\right]\right]\\
&=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\omega^*}_{\pi_t}(X_t^1)+\underbrace{V^{\omega^*}_{\pi^*}(X_t^1)-V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)}_\text{$\leq 0$}\big|\mathcal{H}_t\right]\right]
\end{align*}
where the second term is smaller than zero with the probability that our confidence interval holds through time. Recall the maximum expected cumulative return of each episode is as most $1$, therefore, if we set $\delta(\omega^*) = 1/TP(\omega^*)/P_{\max}$, with $P(\omega^*)$ the prior distribution on $\omega^*$ and $P_{\max}:=\max\lbrace\max_{\omega*}P(\omega^*),1\rbrace$   we can restate the regret as 
\begin{align*}
\textbf{BayesReg}_T:&=1+\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[\phi(X_t^1,\pi_t(X_t^1))^\top \omega(\pi_t)-\phi(X_t^1,\pi_t(X_t^1))^\top \omega^* \big|\mathcal{H}_t\right]\right]\\
&=1+\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[\phi(X_t^1,\pi_t(X_t^1))^\top \left(\wt\omega_t(\pi_t)-\omega^*\right) \big|\mathcal{H}_t\right]\right]
\end{align*}



Again, condition on $\mathcal{H}_t$, and drawn $\mathbf{\Phi}_t$ by following $\pi_t$ we have
\begin{align*}
&\phi(X_t^1,\pi_t(X_t^1))^\top \left(\wt\omega_t(\pi_t)-\omega^*\right)\\
&\quad\quad\quad\quad\quad=\phi(X_t^1,\pi_t(X_t^1))^\top\wo\chi_t^{-1/2}\wo\chi_t^{1/2}\left(\wt\omega_t(\pi_t)-\omega^*\right)\leq \|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\|\wt\omega_t(\pi_t)-\omega^*\|_{\wo\chi_t}
\end{align*}
% \begin{align*}
% &\phi(x_t^1,\pi_t(x_t^1))^\top\omega_t- V^{\omega^*}_{\pi_t}(x_t^1)\\
% &\quad\quad\quad\quad=\mathbbm{1}^\top\mathbf{\Phi}_t\left(\omega_t-\omega^*\right)=\mathbbm{1}^\top\mathbf{\Phi}_t\wo\chi_t^{-1/2}\wo\chi_t^{1/2}\left(\omega_t-\omega^*\right)\leq \sqrt{H} \|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\|\omega_t-\omega^*\|_{\wo\chi_t}
% \end{align*}
Therefore, by running the \PSRL, we get a distribution over the trajectories from episode 1 to $T$
\begin{align*}
\textbf{BayesReg}_T&\leq
1+\E\left[\sum_t^T \|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\|\wt\omega_t(\pi_t)-\omega^*\|_{\wo\chi_t}\right]\\
% &= 
% \E\left[\sum_t^T \|\phi(x_t^1,\pi_t(x_t^1))^\top\|_{\wo\chi_t^{-1}}\|\omega_t-\wh\omega\|_{\wo\chi_t}+\|\phi(x_t^1,\pi_t(x_t^1))^\top\|_{\wo\chi_t^{-1}}\|\omega^*-\wh\omega\|_{\wo\chi_t}\right]\\
&\leq 1+
\E\left[\sum_t^T2\theta_{t-1}(\delta(\omega^*))\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\right]
\end{align*}
Since the maximum expected cumulative reward, given initial the state is at most $1$, we have;
\begin{align*}
\textbf{BayesReg}_T&\leq
1+\E\left[\sum_t^T\min\lbrace2\theta_{t-1}(\delta(\omega^*))\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace\right]\\
&\leq 1+
\E\left[\sum_t^T2\theta_{t-1}(\delta(\omega^*))\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace\right]
\end{align*}
Moreover, at time $T$, we can use Jensen's inequality, exploit the fact that $\theta_t(\delta)$ is an increasing function of $t$ and have
\begin{align}\label{eq:BR1}
\textbf{BayesReg}_T&\leq 1+
\E\left[2\sqrt{T\theta_T(\delta(\omega^*))^2\sum_t^T\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace}\right]\nonumber\\
&\leq 1+
2\left(\sigma\E_{\omega^*}\left[\sqrt{2
\log\left(1/\delta(\omega^*)\right)
+d\log\left(1+TL^2/\lambda\right)}\right]+\lambda^{1/2}L_\omega\right)\nonumber\\
&\quad\quad\quad\quad\quad\quad\quad\E\left[\sqrt{T\sum_t^T\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace}\right]
\end{align}
Using the fact that for any scalar $\alpha$ such that $0\leq \alpha\leq 1$, then $\alpha\leq 2\log(1+\alpha)$, and applying Lemma\ref{lemma:DeterminantLemma} we can rewrite the latter part of Eq.~\ref{eq:BR1}
\begin{align*}
\sqrt{\sum_t^T\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace}\leq 2\sum_t^T\log\left(1+\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\right)
\end{align*}
Also consider 

\begin{align*}
    \E_{\omega^*}\left[\sqrt{2
\log\left(1/\delta(\omega^*)\right)
+d\log\left(1+tL^2/\lambda\right)}\right]
%&\leq    \E_{\omega^*}\left[\sqrt{2/P(\omega^*)}\right]+\sqrt{2\log\left(T/\delta\right)+d\log\left(1+tL^2/\lambda\right)}\\
\leq\sqrt{2/P_{\max}}\mathbbm{H}+\sqrt{2
\log\left(T\right)
+d\log\left(1+tL^2/\lambda\right)}
\end{align*}
where $\mathbbm{H}$ is the differential entropy of the prior. Substituting the RHS of Eq.~\ref{eq:xx} into Eq.~\ref{eq:BR1}, we get 
\begin{align*}
\textbf{BayesReg}_T
&\leq
2\left(\sqrt{2/P_{\max}}\mathbbm{H}\sigma+\sigma\sqrt{2
\log\left(T\right)
+d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2T d\log(\lambda + TL^2/d)}
\end{align*}
which is the the statement in the Theorem.




%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discount factor}
As it clear through the analysis, the only place discount factor appears is in the definitions of
\begin{align*}
\mathbf{\wb R}_t:=\Psi \mathbf{R}_t~~~\wb\nu_t:=\Psi\nu_t
\end{align*}
which does not change the analyses, except through scaling down some of constant factors, e.g., $L_\omega$ and enhancing the regret upper bounds.




==> Sections/old-11-Optimism.tex <==
while $\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t$ is value of $\pi_t$ under model $\beta_t$ at state $x_t^0$ which is also the optimal value at state $x_t^0$ under the model $\beta_t$, $\phi(x_t^0,\pi^*(x_t^0))^\top\beta_t$ is the value of following $\pi^*(x_t^0)$ for one step and then follow $\pi_t$ for the remaining part of horizon. 
Therefore, $\phi(x,\pi_t(x_t^0))^\top\beta_t\geq\phi(x_t^0,\pi^*(x_t^0))^\top\beta_t$. Same argument holds for $\pi^*$ and $\beta^*$, and we also have $\phi(x_t^0,\pi^*(x_t^0))^\top\beta^*\geq\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*$, i.e.  the following inequalities;
\begin{align*}
V_{\beta^*}(x_t^0,\pi_*)=\phi(x_t^0,\pi^*(x_t^0))^\top\beta^* & \geq \phi(x_t^0,\pi_t(x_t^0))^\top\beta^*\\
\phi(x_t^0,\pi^*(x_t^0))^\top\beta_t & \leq V_{\beta_t}(x_t^0,\pi_t)=\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t
\end{align*}

Furthermore, while the value of  $\pi_t$ under  model $\beta^*$  is as follows:

\begin{align*}
V_{\beta^*}(x_t^0,\pi_t)&=\E\left[{r}_{\beta^*}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\beta^*}(x'|x_t^0,\pi_t(x_t^0))V_{\beta^*}(x',\pi_t)\\
&=\E\left[{r}_{\beta^*}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\beta^*}(x'|x_t^0,\pi_t(x_t^0))V_{\beta^*}(x',\pi_t)
\end{align*}

Thanks to these inequalities, we can write the upper bound on the $\textbf{BayesReg}_T$;

\begin{align*}
% \textbf{BayesReg}_T&\leq\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\beta^*}\left[V^{\beta^*}_{\pi^*}(x_t^0)- \beta_t\phi(x_t^0,\pi^*(x_t^0))\big|\mathcal{H}_t\right]\right]+\E_{\mathcal{H}_t}\left[\E_{\beta^*}\left[V^{\beta_t}_{\pi_t}(x_t^0)- V^{\beta^*}_{\pi_t}(x_t^0)\big|\mathcal{H}_t\right]\right]\\ 
% &\quad\quad\quad\quad
\textbf{BayesReg}_T&\leq\sum_t^T \E_{\mathcal{H}_t}\left[ \E_{\beta^*}\left[\underbrace{\phi(x_t^0,\pi^*(x_t^0))^\top\beta^*- \phi(x_t^0,\pi^*(x_t^0))^\top\beta_t}_\text{(a)}\big|\mathcal{H}_t\right]\right]\\
&\quad\quad\quad\quad\quad\quad\quad+\E_{\mathcal{H}_t}\left[\E_{\beta^*}\left[\underbrace{\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t- V^{\beta^*}_{\pi_t}(x_t^0)}_\text{(b)}\big|\mathcal{H}_t\right]\right]
\end{align*}
The first element on the RHS is $(a):\phi(x_t^0,\pi^*(x_t^0))^\top\left(\beta^*-\beta_t\right)$. Since
\begin{align*}
\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*= \E\left[{r}_{\beta^*}(x_t^0,\pi_t(x_t^0))\right]+\int_{x'}T_{\beta^*}(x'|x_t^0,\pi_t(x_t^0))V_{\beta^*}(x',\pi^*)
\end{align*}
the second term can be decomposed as follows;
\begin{align*}
(b):&~\phi(x_t^0,\pi_t(x_t^0))^\top\beta_t-\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*+\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*- V^{\beta^*}_{\pi_t}(x_t^0)\\
&=\phi(x_t^0,\pi_t(x_t^0))^\top\left(\beta_t-\beta^*\right)+\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*- V^{\beta^*}_{\pi_t}(x_t^0)\\
&=\phi(x_t^0,\pi_t(x_t^0))^\top\left(\beta_t-\beta^*\right)+\int_{X^1_t}T_{\beta^*}(X^1_t|x_t^0,\pi_t(x_t^0))\left(\underbrace{V_{\beta^*}(X^1_t,\pi^*)-V_{\beta^*}(X^1_t,\pi_t)}_\text{(c)}\right)
\end{align*}
where $(c)$ can be decomposed the same way as $V_{\beta^*}(x^0_t,\pi^*)-V_{\beta^*}(x^0_t,\pi_t)$. The remaining is to show each of these parts are bounded.
% \begin{align*}
% (c): V_{\beta^*}(x_t^1,\pi^*)-V_{\beta^*}(x_t^1,\pi_t)=\phi(x_t^1,\pi_t(x_t^1))^\top\beta^*-\phi(x_t^1,\pi_t(x_t^))^\top\beta^*+\phi(x_t^0,\pi_t(x_t^0))^\top\beta^*- V^{\beta^*}_{\pi_t}(x_t^0)\\
% \end{align*}
%
\begin{lemma}[Confidence ellipsoid for problem in Eq.~\ref{eq:Bayesian_model}]\label{lem:conf}
For a matrix problem in Eq.~\ref{eq:Bayesian_model}, given a sequence of $\lbrace\mathbf{\Phi}_i,\mathbf{R}_i\rbrace_{i=1}^{t}$, under the Asm.~\ref{asm:subgaussian} and the following estimator for $\wh\beta_t$
\begin{align*}
\wh\beta_t:= \left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\mathbf{R}_i\right)
\end{align*}
with probability at least $1-\delta$
\begin{align*}
\|\wh\beta_t-\beta^*\|_{\wo\chi_t}\leq \sigma\sqrt{2\log\left(\frac{1+tL^2/\lambda}{\delta}\right)}+\lambda^{1/2}L_\beta
\end{align*}
where $\|\beta^*\|_2\leq L_\beta$ and $\|\Psi^{-1}\mathbf{\Phi}(\cdot)\|_2\leq L$. 
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lem:conf}]
Given the estimator $\wh\beta_t$ we have the following:
\begin{align*}
\wh\beta_t&=\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i\beta^* + \nu_i\right)\\
&=\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\\
&+ \left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)\beta^*\\
&-\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\beta^*\\
\end{align*}
therefore, for a given pair of $x,a$
\begin{align*}
\phi(x,a)^\top\wh\beta_t-\phi(x,a)^\top\beta^*&=\phi(x,a)^\top\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\\
&-\phi(x,a)^\top\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\beta^*
\end{align*}
As a results, applying Cauchy–Schwarz inequality and inequalities $\|\beta^*\|_{\wo\chi_t^{-1}}\leq \frac{1}{\lambda\left(\wo\chi_t\right)}\|\beta^*\|_2\leq \frac{1}{\lambda}\|\beta^*\|_2$ we get
\begin{align*}
|\phi(x,a)^\top\wh\beta_t-\phi(x,a)^\top\beta^*|&=\|\phi(x,a)\|_{\wo\chi_t^{-1}}\|\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\|_{\wo\chi_t^{-1}}-\lambda\|\phi(x,a)\|_{\wo\chi_t^{-1}}\|\beta^*\|_{\wo\chi_t^{-1}}\\
&\leq \|\phi(x,a)\|_{\wo\chi_t^{-1}}\|\left(\|\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\nu_i\right)\|_{\wo\chi_t^{-1}}+\lambda^{1/2}\|\beta^*\|_2\right)
\end{align*}
where applying self normalized Lemma \ref{lem:self}, with probability at least $1-\delta$
\begin{align*}
|\phi(x,a)^\top\wh\beta_t-\phi(x,a)^\top\beta^*|\leq \|\phi(x,a)\|_{\wo\chi_t^{-1}}\left(2\sigma\log\left(\frac{\det\left(\wo\chi_t\right)^{1/2}}{\delta\det\left(\wt\chi\right)^{1/2}}\right)+\lambda^{1/2}L_\beta\right)
\end{align*}
hold for any $\phi(x,a)$. By plugging in $\phi(x,a)=\wo\chi_t\left(\wh\beta_t-\beta^*\right)$ %we get the statement in the Lemma \ref{lem:conf}.
we get the following;
\begin{align*}
\|\wh\beta_t-\beta^*\|_{\wo\chi_t}\leq \sigma\sqrt{2\log\left(\frac{\det(\wo\chi_t)^{1/2}\det(\lambda I)^{1/2}}{\delta}\right)}+\lambda^{1/2}L_\beta
\end{align*}
The $\det(\wo\chi_t)$ can be written as $\det(\wo\chi_t)=\Pi_j^d\alpha_j$ therefore, $trace(\wo\chi_t)=\sum_j^d\alpha_j$. We also know that;
\begin{align*}
    (\Pi_j^d\alpha_j)^{1/d}\leq \frac{\sum_j^d\alpha_j}{d}
\end{align*}
Therefore, $\det(\wo\chi_t)\leq \left(\frac{trace(\wo\chi_t)}{d}\right)^d$ while we have $trace(\wo\chi_t)=trace(\lambda I)+\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i\leq d\lambda+tL$, the main statement of Lemma \ref{lem:conf} goes through.
\end{proof}




In order to prove Lemma~\ref{lem:conf}, we need the following Lemma which is a direct extension to the Lemma 10 and 11 in \cite{abbasi-yadkori2011improved}.
\begin{lemma}[Determinant inequality]
For a matrix problem in Eq.~\ref{eq:Bayesian_model}, given a sequence of $\lbrace\mathbf{\Phi}_i,\mathbf{R}_i\rbrace_{i=1}^{t}$, and under $\|\mathbf{\Phi}(\cdot)\|_2\leq L$  we have:
\begin{align*}
\det\left(\wo\chi_t\right)\leq (\lambda+tL^2/d)^d\quad,\quad \sum
\end{align*}
\end{lemma}

% and the value of  $\pi^*$ under  model $\beta_t$  is as follows:

% \begin{align*}
% V_{\beta_t}(x,\pi^*)=\E\left[{r}_{\beta_t}(x,\pi^*(x))\right]+\int_{x'}T_{\beta_t}(x'|x,\pi^*(a))V_{\beta_t}(x',\pi^*)
% \end{align*}

% since

% \begin{align*}
% \beta^*\phi(x,\pi_t(x))= \E\left[{r}_{\beta^*}(x,\pi_t(x))\right]+\int_{x'}T_{\beta^*}(x'|x,\pi_t(x))V_{\beta^*}(x',\pi^*)
% \end{align*}

% and

% \begin{align*}
% \beta_t\phi(x,\pi^*(x))= \E\left[{r}_{\beta_t}(x,\pi^*(x))\right]+\int_{x'}T_{\beta_t}(x'|x,\pi^*(x))V_{\beta_t}(x',\pi_t)
% \end{align*}
% therefore

% since 
% \begin{align*}
% V_{\beta_t}(x,\pi^*)-\beta_t\phi(x,\pi^*(x))= \int_{x'}T_{\beta_t}(x'|x,\pi^*(a))\left(V_{\beta_t}(x',\pi^*)-V_{\beta_t}(x',\pi_t)\right)
% \end{align*}




% \begin{align*}
% V_{\beta^*}(x,\pi_*) & \geq V_{\beta^*}(x,\pi_t)\\
% V_{\beta_t}(x,\pi_*) & \leq V_{\beta_t}(x,\pi_t)
% \end{align*}

% \begin{table*}[h]
%   \centering
%   \footnotesize  
%   \begin{tabular}{ccc}
% %     \multicolumn{1}{c}{}&\multicolumn{12}{c}{} \\
% %     \toprule
%  $V_{\beta^*}(x,\pi_*)$ & $\geq$ & $V_{\beta^*}(x,\pi_t)$ \\
% % \midrule 
% %     \bottomrule
%   \end{tabular}
% \end{table*}


% For a given sequence of states and actions at the episode $t$, $\tau:=\lbrace x^1_t,a^1_t,\ldots,x^H_t,a^H_t\rbrace$ generated under policy $\pi_t$, we are interested in 



% \begin{align*}
% \E_{\mathcal{H}_t}\left[\E_{\beta^*}\left[V^{\beta_t}_{\pi_t}- V^{\beta^*}_{\pi_t}\big|\mathcal{H}_t\right]\right]
% \end{align*}

% the remaining is to show $|V_{\beta^*}(x,\pi_*)-\beta^*\phi(x,\pi_t(x))|$ as well as $|\beta^*\phi(x,\pi^*(x))-\beta_t\phi(x,\pi_t(x)) |$ are  bounded therefore $|V_{\beta^*}(x,\pi_*)-V_{\beta_t}(x,\pi_t)|$ is bounded.






%%%%%%%%%%%%%%%%%%%%%%%%

% \section{not equal}
%  If the $\beta_t$ and $\beta^*$ are not equally distributed conditioned on $\mathbb{H}_t$ we need to show that $\left[\E_{\beta^*}\left[V^{\beta^*}_{\pi^*}- V^{\beta^t}_{\pi_t}\big|\mathcal{H}_t\right]\right] \leq 0$. The posterior distribution over both $\beta^*$ and $\beta_t$, conditioned on the $\mathcal{H}_t$, have the same mean since the likelihood is Gaussian and the prior is same. There is no need to covariance matrices to be equal in order to have the same mean. The choice of the covariance $\mathcal{C}_t$ for $\beta_t$ is designed (using the upper bounds on sub-Gaussian properties of the noises) such that it is wider than the covariance matrix of posterior over $\beta^*$ given the history $\mathcal{C}^*_t$. Therefore, we can rewrite the covariance matrix $\mathcal{C}_t= \mathcal{C}^*_t+A$









==> Sections/old-alter-iclr10-Theory.tex <==
\section{Bayesian and frequentist regrets, Proof of Theorems \ref{Thm:BR} and \ref{Thm:frequentist}}\label{apx:theory}

% \begin{algorithm}[ht]
% \caption{Posterior Sampling Reinforcement Learning}
% \begin{algorithmic}[1]
% \State Input: the prior and likelihood, them construct the posterior
% \For{episode = 1,2,\ldots}
% % 	\State Initialize $x_1$ to the initial State of the environment
%     \State draw $\omega_t$ form posterior
%     \For{$h=0$ to the end of episode}
% 	\State Follow the $\pi_t$, the policy induced by $\omega_t$
% 	\State Update the posterior
% \EndFor
% \EndFor
% \end{algorithmic}
% \label{alg:psrl}
% \end{algorithm}
\paragraph{Modeling:}
We consider the following linear model over the $Q$ functions and returns for episodic MDPs with episode length of $H$. We consider the discount factor to be any number $0\leq \gamma\leq 1$. Let $\omega^*$ denotes the parameter corresponding the underlying model. For a given policy $\pi$ and the time step $h_t$ in the episode, condition on $X^{h_0},A^{h_0}$ we have $\sum_{h=h_0}^H R_h = \phi(X^{h_0},A^{h_0})^\top \omega^*+\sum_{h=h_0}^H \nu_h$ with $\phi(X,A)\in \R^d$. The noise process is correlated, dependent on the agent policy, and is not mean zero unless under policy $\pi^*$.
%
%
\begin{equation}\label{eq:Bayesian_model}
\Psi\mathbf{R} = \mathbf{\Phi}(X^{\{1:H\}},A^{\{1:H\}})\omega^* +\Psi \nu(X^{\{1:H\}},A^{\{1:H\}})~,~~ \textit{where}~,~\Psi:=\left[
  \begin{tabular}{ccccc}
  1 & $\gamma$ & $\gamma^2$ &$\ldots$ & $\gamma^{H-1}$\\
  0 & 1 & $\gamma$ &  $\ldots$ & $\gamma^{H-2}$\\
  0 & 0 & $1$ & $\ldots$ &$\vdots$ \\
  $\vdots$ & $\ldots$ & $\ldots$& $\ldots$ & $\vdots$\\
  $0$ & $\ldots$ & $\ldots$& $\ldots$ & 1
  \end{tabular}
\right]
\end{equation}
The vector $\mathbf{R}\in \Re^H$ is a random vector, as stack of rewards in a episode, i.e., $\mathbf{R}^h = r^h$. The matrix $\mathbf{\Phi}(X^{\{1:H\}},X^{\{1:H\}})\in\Re^{H\times d}$ is a row-wised concatenation of sequence of state-action features, $\mathbf{\Phi}^{h}=\phi(X^h,A^h)$ with $\mathbf{\Phi}_{h}$ denotes the $h$'th row. 

In order to provide more intuition on the model, we can exploit the property of the matrix $\Psi$ where
\begin{align*}
\Psi^{-1}=\left[
  \begin{tabular}{ccccc}
  1 & -$\gamma$ & 0 &$\ldots$ & 0\\
  0 & 1 & -$\gamma$ &  $\ldots$ & 0\\
  0 & 0 & $1$ & $\ldots$ &$\vdots$ \\
  $\vdots$ & $\ldots$ & $\ldots$& $\ldots$ & $\vdots$\\
  $0$ & $\ldots$ & $\ldots$& $\ldots$ & 1
  \end{tabular}
\right]
\end{align*}
and rewrite Eq.~\ref{eq:Bayesian_model} as follows:

\begin{equation}
\mathbf{R}_t = \Psi^{-1}\mathbf{\Phi}_t\omega + \nu_t
\end{equation}
We denote $\Psi':={\Psi^{-1}}^\top$.
We build our analysis based on the former notation. We consider the feature representing matrix and weights for any $X^{\{1:H\}},A^{\{1:H\}}$ to satisfy;
\begin{align*}
    trace\left(\mathbf{\Phi}(X^{\{1:H\}},A^{\{1:H\}})^\top \Psi'\Psi^{-1}\mathbf{\Phi}(X^{\{1:H\}},A^{\{1:H\}})\right)\leq L~,~\|\omega\|_2\leq L_\omega
\end{align*}
The vector $\nu(X^{\{1:H\}},A^{\{1:H\}})\in\Re^H$
is a state-action and policy dependent noise vector. The MDP assumption is crucial for the analysis in this paper. The noise $\nu^{h}$ encodes the randomness in transition to state $X^h$, possible stochasticity in policy i.e., $A^h$, reward $R^h$. For any $h$, the noises after time step $h$, $\lbrace\nu^{h},\nu^{h+1},\ldots, \nu^{H}\rbrace$, are conditionally independent from the noises before time step $h'$, $\lbrace\nu^{1},\nu^{2},\ldots, \nu^{h-1}\rbrace$ given $(X^h,A^h)$. Moreover, since $\nu^{h}$ encodes the stochasticity in transition and reward at time step $h$, conditional distribution of $\nu^{h}|(X^h,A^h)$ is mean zero and independent $\lbrace\nu^{0},\ldots\lbrace\nu^{h-1},\nu^{h+1},\ldots, \nu^{H}\rbrace$ other of since $\phi(X^h,A^h)^\top\omega^*$ represent the true $Q$ value of $X^h,A^h$. 


The agent policy at each episode is denoted as $\pi_t$. In the remaining, we show how to estimate $\omega^*$ through data collected by following  $\pi_t$. We denote $\hat{\omega}_t$, the estimation of $\omega^*$. We show over time the estimation concentrates around $\omega^*$ under the desire matrix norm. We further show, we can deploy this analysis an construct two algorithms, one based on \PSRL, and another Optimism \OFU to guaranteed Bayesian and frequentist regret upper bounds respectively. The main body of the following analyses on concentration of measure is a matrix extension of  contextual linear bandit analyses ~\cite{abbasi-yadkori2011improved,chu2011contextual,li2010contextual,rusmevichientong2010linearly,dani2008stochastic,russo2014learning} and self normalized processes~\citep{de2004self}. Our regret analysis extends prior analysis in frequentist and Bayesian regret literature~\cite{osband2013more,jaksch2010near}.

We restate the Eq.~\ref{eq:Bayesian_model} in its abstract way;
\begin{equation}
\mathbf{\wb R}_t:=\Psi \mathbf{R}_t=\mathbf{\Phi}_t\omega + \wb\nu_t~,~~~\textit{where}~~~\wb\nu_t:=\Psi\nu_t
\end{equation}
% \eb{This is a bit unclear. Is this an assumption on the model of the environment, or a particular representation/decomposition that is independent of the domain?}
We consider the discount factor to be any number $0\leq \gamma\leq 1$ for the modeling and for the sake of analysis we consider $\gamma=1$ from now on which we later argue the bounds also hold for any $0\leq \gamma\leq 1$.



% \input{Sections/diagram.tex}

\begin{assumption}[Sub-Gaussian random vector \citep{hsu2012tail}]\label{asm:subgaussian}
The noise model at time $t$, conditioned on the filtration $\F_{t-1}$ at time $t$ is sub-Gaussian random vector, i.e. there exists a parameter $\sigma\geq 0$ such that $\forall \alpha\in\R^d$
\begin{align*}
\E\left[\exp\left(\alpha^\top \wb\nu_t\right)\Big|\F_{t-1}\right]\leq \exp\left(\|\alpha\|_2\sigma^2/2\right)
\end{align*}
\end{assumption}
The filtration at time t also includes $X^{\{1:H\}},A^{\{1:H\}}$. Asm.~\ref{asm:subgaussian} also implies that $\E\left[\wb\nu_t\Big|\F_{t}\right]=0$ which means that after drawing the matrix $\mathbf{\Phi}_t$, the random variable $\wb\nu_t$ is means zero.
A similar assumption on the noise model is assumed in prior analyses of linear bandit \citep{abbasi-yadkori2011improved}.

Furthermore, we consider the maximum expected cumulative reward condition on states of a episode is at most $1$.

Defined the following quantities for self-normalized processes;
\begin{align*}
S_t := \sum_i^t \mathbf{\Phi}_i^\top\Psi'\nu_i, ~~~~~ \chi_t := \sum_{i=1}^t  \mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i, ~~~~~ \wo\chi_t = \chi_t+\wt\chi
\end{align*}
where $\wt\chi$ is a ridge regularization matrix and usually is equal to $\lambda I$. 
% Let's denote $\tau$ as the stopping time.

\begin{lemma}[Confidence ellipsoid for problem in Eq.~\ref{eq:Bayesian_model}]\label{lem:conf}
For a matrix problem in Eq.~\ref{eq:Bayesian_model}, given a sequence of $\lbrace\mathbf{\Phi}_i,\mathbf{R}_i\rbrace_{i=1}^{T}$, under the Asm.~\ref{asm:subgaussian} and the following estimator for $\wh\omega_t$
\begin{align*}
\wh\omega_t:= \left(\sum_i^t\mathbf{\Phi}_i^\top\Psi'\Psi^{-1}\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\Psi'\mathbf{R}_i\right)
\end{align*}
with probability at least $1-\delta$
\begin{align*}
\|\wh\omega_\tau-\omega^*\|_{\wo\chi_t}\leq\theta_t(\delta)&:\sigma\sqrt{2
\log\left(1/\delta\right)
+d\log\left(1+tL^2/\lambda\right)}+\lambda^{1/2}L_\omega
% &\leq \sigma\sqrt{2
% \log\left(1/\delta\right)
% +d\log\left(1+tL^2/\lambda\right)}+\lambda^{1/2}L_\omega
\end{align*}
for all $t\leq T$ where $\|\omega^*\|_2\leq L_\omega$ and $trace{\left(\mathbf{\Phi}(\cdot)\mathbf{\Phi}(\cdot)^\top\right)}\leq L$, and therefore the confidence set is
\begin{align*}
    \C_t(\delta):=\lbrace\omega\in\Re^d:\|\wh\omega_t-\omega\|_{\wo\chi_t}\leq \theta_t(\delta)\rbrace
\end{align*}
\end{lemma}

Let $\Theta_T$ denote the event that the confidence bounds in Lemma~\ref{lem:conf} holds.
\begin{lemma}[Determinant Lemma]\label{lemma:DeterminantLemma}
For a sequence $\sum_t^T\log\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}\right)$ we have
\begin{align}\label{eq:xx}
\sum_t^T\log\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}\right)\leq d\log(\lambda + TL^2/d)
\end{align}
\end{lemma}

\paragraph{Regret Definition}
We defined $V^{\omega}_{\pi}$, the value of policy $\pi$ applied on model specified by $\omega$ in Eq.~\ref{eq:Bayesian_model}. We restate the definition of the regret and Bayesian regret.
\begin{align*}
\textbf{Reg}_T:&=\E\left[\sum_t^T \left[V^{\omega^*}_{\pi^*}-V^{\omega^*}_{\pi_t}\right]|\omega^*\right]
\end{align*}
Where  $\pi_t$ is the agent policy at time $t$
%the policy induced by $\omega^t$, $\pi_t(x,a)=\arg\max_{a'}\omega_t\phi(x,a')$. 

When there is a prior over the $\omega^*$  the expected Bayesian regret might be the target of the study. 
\begin{align*}
\textbf{BayesReg}_T:&=\E\left[\sum_t^T \left[V^{\omega^*}_{\pi^*}-V^{\omega^*}_{\pi_t}\right]\right]
%
% &=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(X_t^1)\big|\mathcal{H}_t\right]\right]\\
%
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Optimism: Regret bound of Alg.~\ref{alg:optimism}}\label{sub:optimism}


Given samples by following the agent policy $\pi_t'$ for each episode $t'\leq t$ we estimate the $\wh \omega_t$ as follows; 
\begin{align*}
\wh\omega_t:= \left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\mathbf{\wb R}_i\right)
\end{align*}
Lemma~\ref{lem:conf} states that under event $\Theta_T$, $\|\wh\omega_t-\omega^*\|_{\wo\chi_t}\leq\theta_t(\delta)$. For an observed state $X_t^1$, the optimistic policy is

\begin{align*}
    \wt\pi_t(X_t^h)=\arg\max_{a\in\A}\max_{\omega\in\C_{t-1}(\delta)}\phi^\top(X_t^h,a)\omega
\end{align*}
Furthermore, we define state and policy dependent optimistic parameter  $\wt\omega_t(\pi)$ as follows;
\begin{align*}
\wt\omega_t(\pi):=\arg\max_{\omega\in \C_{t-1}(\delta)}\phi(X_t^1,\pi(X_t^1))^\top\omega
\end{align*}
For ease of notation we drop the state in the notation. Following \OFU, Alg.~\ref{alg:optimism}, we set $\pi_t=\wt\pi_t$ denote the optimistic policy. By the definition we have
\begin{align*}
    V^{\wt\omega_t(\wt\pi_t)}_{\wt\pi_t}(X_t^h)\geq V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^h)
\end{align*}
Therefore, under the event $\Theta_T$ we have

\begin{align*}
\textbf{Reg}_T:&=\E\left[\sum_t^T\left[\underbrace{V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\wt\pi_t}(X_t^1)}_{\Delta_t^{h=1}}\right]|\omega^*\right]\\
&\leq\E \left[\sum_t^T\left[V^{\wt\omega_t(\wt\pi_t)}_{\wt\pi_t}(X_t^1)-V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)+V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\wt\pi_t}(X_t^1)\right]|\omega^*\right]\\
&=\E\left[\sum_t^T \left[V^{\wt\omega_t(\wt\pi_t)}_{\wt\pi_t}(X_t^1)-V^{\omega^*}_{\wt\pi_t}(X_t^1)+\underbrace{V^{\omega^*}_{\pi^*}(X_t^1)-V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)}_\text{$\leq 0$}\right]|\omega^*\right]\\
% &=\sum_t^T V^{\wt\omega_t}_{\wt\pi_t}(x_t^1)-V^{\omega^*}_{\wt\pi_t}(x_t^1)%=\sum_t^T\phi(x_t^1,\wt\pi_t(x_t^1))^\top \left(\wt\omega_t-\omega^*\right)
\end{align*}
Resulting in 
\begin{align*}
\textbf{Reg}_T&\leq\E\left[\sum_t^T\left[ V^{\wt\omega_t(\wt\pi_t)}_{\wt\pi_t}(X_t^1)-V^{\omega^*}_{\wt\pi_t}(X_t^1)\right]|\omega^*\right]
%=\sum_t^T\phi(x_t^1,\wt\pi_t(x_t^1))^\top \left(\wt\omega_t-\omega^*\right)
\end{align*}
Lets defined $V^{\omega}_{\pi}(X_t^1,\ldots, X_t^{h'};h:\pi')$ as the value function following policy $\pi$ for $h$ time step then switching to policy $\pi'$ on the model $\omega$ and observing $X_t^1,\ldots X_t^{h'}$.
\begin{align*}
\textbf{Reg}_T&\leq\E\left[\sum_t^T \left[V^{\wt\omega_t(\wt\pi_t)}_{\wt\pi_t}(X_t^1)-V^{\omega^*}_{\wt\pi_t}(X_t^1)\right]|\omega^*\right]\\
&=\E\left[\sum_t^T \left[V^{\wt\omega_t(\wt\pi_t)}_{\wt\pi_t}(X_t^1)-V^{\omega^*}_{\wt\pi_t}(X_t^1;1:\pi^*)+V^{\omega^*}_{\wt\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\wt\pi_t}(X_t^1)\right]|\omega^*\right]
%=\sum_t^T\phi(x_t^1,\wt\pi_t(x_t^1))^\top \left(\wt\omega_t-\omega^*\right)
\end{align*}
Given the generative model in Eq.\ref{eq:Bayesian_model} we have
\begin{align*}
\textbf{Reg}_T&\leq\E\left[\sum_t^T\left[ V^{\wt\omega_t(\wt\pi_t)}_{\wt\pi_t}(X_t^1)-V^{\omega^*}_{\wt\pi_t}(X_t^1;1:\pi^*)+V^{\omega^*}_{\wt\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\wt\pi_t}(X_t^1)\right]|\omega^*\right]\\
&=\E\left[\sum_t^T \left[\phi(X_t^1,\wt\pi_t(X_t^1))^\top\wt\omega_t(\wt\pi_t)-\phi(X_t^1,\wt\pi_t(X_t^1))^\top\omega^*+V^{\omega^*}_{\wt\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\wt\pi_t}(X_t^1)\right]|\omega^*\right]\\
&=\E\left[\sum_t^T \left[\phi(X_t^1,\wt\pi_t(X_t^1))^\top\left(\wt\omega_t(\wt\pi_t)-\omega^*\right)+\underbrace{V^{\omega^*}_{\wt\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\wt\pi_t}(X_t^1)}_{(\Delta_t^{h=2})}\right]|\omega^*\right]
%=\sum_t^T\phi(x_t^1,\wt\pi_t(x_t^1))^\top \left(\wt\omega_t-\omega^*\right)
\end{align*}
% V^{\omega^*}_{\wt\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\wt\pi_t}(X_t^1)
For $\Delta_t^{h=2}$ we deploy the similar decomposition and upper bound as $\Delta_t^{h=1}$
\begin{align*}
\Delta_t^2:=V^{\omega^*}_{\wt\pi_t}(X_t^1;1:\pi^*)-V^{\omega^*}_{\wt\pi_t}(X_t^1)
\end{align*}
Since for both of $V^{\omega^*}_{\wt\pi_t}(X_t^1;1:\pi^*)$ and $V^{\omega^*}_{\wt\pi_t}(X_t^1)$ we follow the same policy on the same model for 1 time step, the reward at the first time step has the same distribution, therefore we have;
\begin{align*}
\Delta_t^{h=2}&=E\left[V^{\omega^*}_{\wt\pi_t}(X_t^2;1:\pi^*)-V^{\omega^*}_{\wt\pi_t}(X_t^2)|X_t^1,\omega^*\right]
\end{align*}
rustling in 
\begin{align*}
\Delta_t^{h=2}&=E\left[V^{\omega^*}_{\wt\pi_t}(X_t^2;1:\pi^*)-V^{\omega^*}_{\wt\pi_t}(X_t^2)|X_t^1,\omega^*\right]\\
&\leq\E\left[\phi(X_t^2,\wt\pi_t(X_t^2))^\top\left(\wt\omega_t(\wt\pi_t)-\omega^*\right)+\underbrace{V^{\omega^*}_{\wt\pi_t}(X_t^2;2:\pi^*)-V^{\omega^*}_{\wt\pi_t}(X_t^2)}_{(\Delta_t^{h=3})}|X_t^1,\omega^*\right]
\end{align*}
Similarly we can defined $\Delta_t^{h=3}, \ldots \Delta_t^{h=H}$. Therefore;


\begin{align}\label{eq:onesnorm}
\textbf{Reg}_T&\leq\E\left[\sum_t^T\sum_h^H \phi(X_t^h,\wt\pi_t(X_t^h))^\top\left(\wt\omega_t(\wt\pi_t)-\omega^*\right)|\omega^*\right]\nonumber\\
&=\E\left[\sum_t^T\mathbbm{1}^\top\mathbf{\Phi}_t\left(\wt\omega_t(\wt\pi_t)-\omega^*\right)|\omega^*\right]\nonumber\\
&=\E\left[\sum_t^T\mathbbm{1}^\top\mathbf{\Phi}_t\wo\chi_{t-1}^{-1/2}\wo\chi_{t-1}^{1/2}\left(\wt\omega_t(\wt\pi_t)-\omega^*\right)|\omega^*\right]\nonumber\\
&\leq  \E\left[\sqrt{H}\sum_t^T \|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}\|\wt\omega_t(\wt\pi_t)-\omega^*\|_{\wo\chi_{t-1}}|\omega^*\right]\nonumber\\
&\leq \E\left[\sqrt{H}\sum_t^T \|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}2\theta_{t-1}(\delta)|\omega^*\right]
\end{align}

Since the maximum expected cumulative reward, condition on states of a episode is at most $1$, we have;
\begin{align*}
\textbf{Reg}_T&\leq\sqrt{H}\E\left[\sum_t^T \min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}2\theta_{t-1}(\delta),1\rbrace|\omega^*\right]\\
&\leq\sqrt{H}\E\left[\sum_t^T\sum_h^H2\theta_{t-1}(\delta) \min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}},1\rbrace|\omega^*\right]\\
\end{align*}


Moreover, at time $T$, we can use Jensen's inequality, exploit the fact that $\theta_t(\delta)$ is an increasing function of $t$ and have

\begin{align}\label{eq:OR1}
\textbf{Reg}_T&\leq2\E\left[\sqrt{TH\theta_{T}(\delta)^2\sum_t^T \min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}},1\rbrace}|\omega^*\right]\nonumber\\
&\leq 
2\left(\sigma\sqrt{2
\log\left(1/\delta\right)
+d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\E\left[\sqrt{TH\sum_t^T\min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}},1\rbrace}|\omega^*\right]
\end{align}

Now, using the fact that for any scalar $\alpha$ such that $0\leq \alpha\leq 1$, then $\alpha\leq 2\log(1+\alpha)$ we can rewrite the latter part of Eq.~\ref{eq:OR1}
\begin{align*}
\sqrt{\sum_t^T\min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}},1\rbrace}\leq 2\sum_t^T\log\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_{t-1}^{-1}}\right)
\end{align*}
By applying the Lemma~\ref{lemma:DeterminantLemma} and substituting the RHS of Eq.~\ref{eq:xx} into Eq.~\ref{eq:OR1}, we get 
\begin{align}\label{eq:regOPT}
\textbf{Reg}_T
&\leq
2\left(\sigma\sqrt{2
\log\left(1/\delta\right)
+d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2TH d\log(\lambda + TL^2/d)}
\end{align}
with probability at least $1-\delta$. If we set $\delta=1/T$ then the probability that the event $\Theta_T$ holds is $1-1/T$ and we get regret of at most the RHS of Eq.~\ref{eq:regOPT}, otherwise with probability at most $1/T$ we get maximum regret of $T$, therefore 
\begin{align*}
\textbf{Reg}_T
&\leq 1+
2\left(\sigma\sqrt{2
\log\left(T\right)
+d\log \left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2THd\log(\lambda + TL^2/d)}
\end{align*}
and theorem statement follows.






% \begin{align*}
% \textbf{Reg}_T&\leq2\E\left[\sqrt{TH\theta_{T}(\delta)^2\sum_t^T \min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_t^-1},1\rbrace}|\omega^*\right]\nonumber\\
% &\leq 
% \left(2\sigma\sqrt{2
% \log\left(1/\delta\right)
% +d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\E\left[\sqrt{TH\sum_t^T\min\lbrace\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}},1\rbrace}|\omega^*\right]
% \end{align*}


% \begin{align}%\label{eq:BR1}
% \textbf{Reg}_T&\leq2 \sqrt{T\theta_T(\delta)^2\sum_t^T\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace}\nonumber\\
% &\leq 
% \left(2\sigma\sqrt{2
% \log\left(1/\delta\right)
% +d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\nonumber\\
% &\quad\quad\quad\quad\quad\quad\quad\sqrt{T\sum_t^T\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace}
% \end{align}
% Now, using the fact that for any scalar $\alpha$ such that $0\leq \alpha\leq 1$, then $\alpha\leq 2\log(1+\alpha)$ we can rewrite the latter part of Eq.~\ref{eq:BR1}
% \begin{align*}
% \sqrt{\sum_t^T\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace}\leq 2\sum_t^T\log\left(1+\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\right)
% \end{align*}
% Substituting the RHS of Eq.~\ref{eq:xx} into Eq.~\ref{eq:BR1}, we get 
% \begin{align*}
% \textbf{Reg}_T
% &\leq
% 2\left(\sigma\sqrt{2
% \log\left(1/\delta\right)
% +d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2T d\log(\lambda + TL^2/d)}
% \end{align*}
% with probability at least $1-\delta$. If we $\delta=1/T$ we get
% \begin{align*}
% \textbf{Reg}_T
% &\leq
% 2\left(\sigma\sqrt{2
% \log\left(T\right)
% +d\log \left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2T d\log(\lambda + TL^2/d)}
% \end{align*}
% and theorem statement follows.
% % \begin{align*}
% % \textbf{Reg}_T:&=\sum_t^T V^{\omega^*}_{\pi^*}- V^{\omega^*}_{\wt\pi_t}\leq \left(\sigma\sqrt{2
% % \log\left(1/\delta\right)
% % +d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2T d\log(\lambda + TL^2/d)}
% % \end{align*}
% % with probability at least $1-\delta$, and  with $\delta=1/T$ the theorem follows.

%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{Sections/11-Bayesian.tex}

\input{Sections/12-Lemmas.tex}
% \subsection{Bayesian Regret}\label{sec:proof}
% The analysis developed in the previous section, up to some minor modification,  directly apply to Bayesian regret bound, when \PSRL is considered.

% When there is a prior over the $\omega^*$  the expected Bayesian Regret might be target of study. 
% \begin{align*}
% \textbf{BayesReg}_T:&=\E_{\omega^*}\left[\textbf{Reg}_T\right]:=\E_{\omega*}\left[\sum_t^T V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(X_t^1)\right]\\
% %
% &=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(X_t^1)\big|\mathcal{H}_t\right]\right]\\
% %
% \end{align*}
% Here $\mathcal{H}_t$ is a multivariate random sequence which indicates history at the beginning of episode $t$, including $X_t^1$ and  $\omega_t$ is the model parameter chosen through \PSRL. 

% Condition on the history $\mathcal{H}_t$, we estimate the $\wh \omega_t$ as follows; 
% \begin{align*}
% \wh\omega_t:= \left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\mathbf{\wb R}_i\right)
% \end{align*}
% Lemma~\ref{lem:conf} states that with probability at least $1-\delta$, 
% $\|\wh\omega_t-\omega^*\|_{\wo\chi_t}\leq\theta_t(\delta)$, $\forall t\leq \tau$. Let construct the confidence interval as follows;
% The confidence set $\C_t(\delta)$, condition on $\mathcal{H}_t$ is deterministic. Following \PSRL Alg.~\ref{alg:psrl}, we set $\pi_t$ drawn from the posterior distribution.

% Conditioned on $\mathcal{H}_t$, the $\omega_t$ and $\omega^*$ are equally distributed, then we have
% \begin{align*}
%  \E_{\omega_*}\left[V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)\big|\mathcal{H}_t\right]=\E_{\omega_*}\left[ V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)\big|\mathcal{H}_t\right]   
% \end{align*}
% therefore, resulting in
% \begin{align*}
% \textbf{BayesReg}_T:&=\E_{\omega^*}\left[\textbf{Reg}_T\right]:=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(x_t^1)\big|\mathcal{H}_t\right]\right]\\
% %
% &=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)+V^{\omega^*}_{\pi^*}(X_t^1)- V^{\omega^*}_{\pi_t}(X_t^1)\big|\mathcal{H}_t\right]\right]\\
% &=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[V^{\wt\omega_t(\pi_t)}_{\pi_t}(X_t^1)-V^{\omega^*}_{\pi_t}(X_t^1)+\underbrace{V^{\omega^*}_{\pi^*}(X_t^1)-V^{\wt\omega_t(\pi^*)}_{\pi^*}(X_t^1)}_\text{$\leq 0$}\big|\mathcal{H}_t\right]\right]
% \end{align*}
% where the second term is smaller than zero with the probability that our confidence interval holds through time. Recall the maximum expected cumulative return of each episode is as most $1$, therefore, if we set $\delta(\omega^*) = 1/TP(\omega^*)/P_{\max}$, with $P(\omega^*)$ the prior distribution on $\omega^*$ and $P_{\max}:=\max\lbrace\max_{\omega*}P(\omega^*),1\rbrace$   we can restate the regret as 
% \begin{align*}
% \textbf{BayesReg}_T:&=1+\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[\phi(X_t^1,\pi_t(X_t^1))^\top \omega(\pi_t)-\phi(X_t^1,\pi_t(X_t^1))^\top \omega^* \big|\mathcal{H}_t\right]\right]\\
% &=1+\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[\phi(X_t^1,\pi_t(X_t^1))^\top \left(\wt\omega_t(\pi_t)-\omega^*\right) \big|\mathcal{H}_t\right]\right]
% \end{align*}



% Again, condition on $\mathcal{H}_t$, and drawn $\mathbf{\Phi}_t$ by following $\pi_t$ we have
% \begin{align*}
% &\phi(X_t^1,\pi_t(X_t^1))^\top \left(\wt\omega_t(\pi_t)-\omega^*\right)\\
% &\quad\quad\quad\quad\quad=\phi(X_t^1,\pi_t(X_t^1))^\top\wo\chi_t^{-1/2}\wo\chi_t^{1/2}\left(\wt\omega_t(\pi_t)-\omega^*\right)\leq \|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\|\wt\omega_t(\pi_t)-\omega^*\|_{\wo\chi_t}
% \end{align*}
% % \begin{align*}
% % &\phi(x_t^1,\pi_t(x_t^1))^\top\omega_t- V^{\omega^*}_{\pi_t}(x_t^1)\\
% % &\quad\quad\quad\quad=\mathbbm{1}^\top\mathbf{\Phi}_t\left(\omega_t-\omega^*\right)=\mathbbm{1}^\top\mathbf{\Phi}_t\wo\chi_t^{-1/2}\wo\chi_t^{1/2}\left(\omega_t-\omega^*\right)\leq \sqrt{H} \|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\|\omega_t-\omega^*\|_{\wo\chi_t}
% % \end{align*}
% Therefore, by running the \PSRL, we get a distribution over the trajectories from episode 1 to $T$
% \begin{align*}
% \textbf{BayesReg}_T&\leq
% 1+\E\left[\sum_t^T \|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\|\wt\omega_t(\pi_t)-\omega^*\|_{\wo\chi_t}\right]\\
% % &= 
% % \E\left[\sum_t^T \|\phi(x_t^1,\pi_t(x_t^1))^\top\|_{\wo\chi_t^{-1}}\|\omega_t-\wh\omega\|_{\wo\chi_t}+\|\phi(x_t^1,\pi_t(x_t^1))^\top\|_{\wo\chi_t^{-1}}\|\omega^*-\wh\omega\|_{\wo\chi_t}\right]\\
% &\leq 1+
% \E\left[\sum_t^T2\theta_{t-1}(\delta(\omega^*))\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\right]
% \end{align*}
% Since the maximum expected cumulative reward, given initial the state is at most $1$, we have;
% \begin{align*}
% \textbf{BayesReg}_T&\leq
% 1+\E\left[\sum_t^T\min\lbrace2\theta_{t-1}(\delta(\omega^*))\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace\right]\\
% &\leq 1+
% \E\left[\sum_t^T2\theta_{t-1}(\delta(\omega^*))\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace\right]
% \end{align*}
% Moreover, at time $T$, we can use Jensen's inequality, exploit the fact that $\theta_t(\delta)$ is an increasing function of $t$ and have
% \begin{align}\label{eq:BR1}
% \textbf{BayesReg}_T&\leq 1+
% \E\left[2\sqrt{T\theta_T(\delta(\omega^*))^2\sum_t^T\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace}\right]\nonumber\\
% &\leq 1+
% 2\left(\sigma\E_{\omega^*}\left[\sqrt{2
% \log\left(1/\delta(\omega^*)\right)
% +d\log\left(1+TL^2/\lambda\right)}\right]+\lambda^{1/2}L_\omega\right)\nonumber\\
% &\quad\quad\quad\quad\quad\quad\quad\E\left[\sqrt{T\sum_t^T\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace}\right]
% \end{align}
% Using the fact that for any scalar $\alpha$ such that $0\leq \alpha\leq 1$, then $\alpha\leq 2\log(1+\alpha)$, and applying Lemma\ref{lemma:DeterminantLemma} we can rewrite the latter part of Eq.~\ref{eq:BR1}
% \begin{align*}
% \sqrt{\sum_t^T\min\lbrace\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}},1\rbrace}\leq 2\sum_t^T\log\left(1+\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\right)
% \end{align*}
% Also consider 

% \begin{align*}
%     \E_{\omega^*}\left[\sqrt{2
% \log\left(1/\delta(\omega^*)\right)
% +d\log\left(1+tL^2/\lambda\right)}\right]
% %&\leq    \E_{\omega^*}\left[\sqrt{2/P(\omega^*)}\right]+\sqrt{2\log\left(T/\delta\right)+d\log\left(1+tL^2/\lambda\right)}\\
% \leq\sqrt{2/P_{\max}}\mathbbm{H}+\sqrt{2
% \log\left(T\right)
% +d\log\left(1+tL^2/\lambda\right)}
% \end{align*}
% where $\mathbbm{H}$ is the differential entropy of the prior. Substituting the RHS of Eq.~\ref{eq:xx} into Eq.~\ref{eq:BR1}, we get 
% \begin{align*}
% \textbf{BayesReg}_T
% &\leq
% 2\left(\sqrt{2/P_{\max}}\mathbbm{H}\sigma+\sigma\sqrt{2
% \log\left(T\right)
% +d\log\left(1+TL^2/\lambda\right)}+\lambda^{1/2}L_\omega\right)\sqrt{2T d\log(\lambda + TL^2/d)}
% \end{align*}
% which is the the statement in the Theorem.




% %%%%%%%%%%%%%%%%%%%%%%
% \subsection{Discount factor}
% As it clear through the analysis, the only place discount factor appears is in the definitions of
% \begin{align*}
% \mathbf{\wb R}_t:=\Psi \mathbf{R}_t~~~\wb\nu_t:=\Psi\nu_t
% \end{align*}
% which does not change the analyses, except through scaling down some of constant factors, e.g., $L_\omega$ and enhancing the regret upper bounds.






% \subsection{Proof of Lemmas}

% \begin{lemma}\label{lem:M_t}
% Let $\alpha\in\R^d$ be be an arbitrary vector and for any $t\geq0$ define
% \begin{align*}
% M_t^\alpha :=\exp\left(\sum_i^t\left[\frac{\alpha^\top \mathbf{\Phi}_i^\top\wb\nu_i}{\sigma}-\frac{1}{2}\|\mathbf{\Phi_i}\alpha\|^2_2\right]\right)
% \end{align*}
% Then, for a stopping time under the filtration $\{\F_t\}_{t=0}^\infty$, $M_\tau^\lambda\leq 1$.
% \end{lemma}



% \begin{proof}~Lemma.~\ref{lem:M_t}
% We first show that $\{M_t^\alpha\}_{t=0}^\infty$ is a supermartingale sequence. Let
% \begin{align*}
% D_i^\alpha = \exp\left(\frac{\alpha^\top \mathbf{\Phi}_i^\top\wb\nu_i}{\sigma}-\frac{1}{2}\|\mathbf{\Phi_i}\alpha\|^2_2\right)
% \end{align*}
% Therefore, we can rewrite $\E\left[M^\alpha_t\right]$ as follows:
% \begin{align*}
% \E\left[M_t^\alpha|\F_{t-1}\right] = \E\left[D_1^\alpha\ldots D_{t-1}^\alpha D_{t}^\alpha|\F_{t-1}\right] = D_1^\alpha\ldots D_{t-1}^\alpha\E\left[ D_{t}^\alpha|\F_{t-1}\right]\leq M_{t-1}^\alpha
% \end{align*}
% The last inequality follows since $\E\left[ D_{t}^\alpha|\F_{t-1}\right]\leq 1$ due to Assumption~\ref{asm:subgaussian}, therefore since for the first time step $\E\left[M_1^\alpha\right]\leq 1$, then $\E\left[M_t^\alpha\right]\leq 1$. For a stopping time $\tau$, Define a variable $\wo{M}_t^\alpha = M_{\min\{t,\tau\}}^\alpha$ and since $\E\left[M_\tau^\alpha\right]= \E\left[\lim\inf_{t\rightarrow\infty}\wo{M}_t^\alpha\right]\leq \lim\inf_{t\rightarrow \infty}\E\left[\wo{M}_t^\alpha\right]\leq 1$, therefore the Lemma.~\ref{lem:M_t} holds.
% \end{proof}

% % Let's defined the following quantities for self-normalized processes;
% % \begin{align*}
% % S_t := \sum_i^t \mathbf{\Phi}_i^\top\wb\nu_i, ~~~~~ \chi_t := \sum_{i=0}^t  \mathbf{\Phi}_i^\top\mathbf{\Phi}_i, ~~~~~ \wo\chi_t = \chi_t+\wt\chi
% % \end{align*}
% % where $\wt\chi$ is a ridge regularization matrix and usually is equal to $\lambda I$.
% \begin{lemma} \label{lem:self}[Extension to Self-normalized bound in \cite{abbasi-yadkori2011improved}] For a stopping time $\tau$ and filtration $\{\F_t\}_{t=0}^\infty$, with probability at least $1-\delta$
% \begin{align*}
% \|S_\tau\|_{\wo\chi_\tau^{-1}}\leq 2\sigma^2\log(\frac{\det\left(\wo\chi_t\right)^{1/2}\det(\wt\chi)^{-1/2}}{\delta})
% \end{align*}
% \end{lemma}
% \begin{proof}~Lemma.~ \ref{lem:self}
% Given the definition of the parameters of self-normalized process, we can rewrite $M_t^\alpha$ as follows;
% \begin{align*}
% M_t^\alpha = \exp\left(\frac{\alpha^\top S_t}{\sigma}-\frac{1}{2}\|\alpha\|_{\chi_t}\right)
% \end{align*}
% Consider $\Omega$ as a Gaussian random vector, denoted as $f(\Omega=\alpha)$, with covariance matrix of $\wo \chi^{-1}$. Define $M_t:=\E\left[M_t^\Omega|\F_\infty\right]$, which also results in $\E\left[M_t\right]=\E\left[\E\left[M_t^\Omega|\Omega\right]\right]\leq 1$. Therefore
% \begin{align*}
% M_t=&\int_{\Re^d}\exp\left(\frac{\alpha^\top S_t}{\sigma}-\frac{1}{2}\|\alpha\|_{\chi_t}\right)f(\alpha)d\alpha\\
% %
% =&\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\frac{1}{2}\|S_t/\sigma\|^2_{\chi_t^{-1}}\right)f(\alpha)d\alpha\\
% %
% =&\sqrt{\frac{\det\left(\wt\chi\right)}{\left(2\pi\right)^d}}\exp\left(\frac{1}{2}\|S_t/\sigma\|_{\chi_t^{-1}}\right)\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\frac{1}{2}\|\alpha\|^2_{\wt\chi}\right)d\alpha
% \end{align*}
% Since $\chi_t$ and $\wt\chi$ are positive semi definite and positive definite respectively, we have 
% \begin{align*}
% \|\alpha-\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}+\|\alpha\|^2_{\wt\chi}&= \|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}+\|\chi_t^{-1}S_t/\sigma\|^2_{\chi_t}-\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}\\
% &=\|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}+\|\S_t/\sigma\|^2_{\chi_t^{-1}}-\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}
% \end{align*}
% Therefore, 
% \begin{align*}
% M_t=&\sqrt{\frac{\det\left(\wt\chi\right)}{\left(2\pi\right)^d}}\exp\left(\frac{1}{2}\|S_t/\sigma\|_{\left(\wt\chi+\chi_t\right)^{-1}}\right)\int_{\Re^d}\exp\left(\frac{1}{2}\|\alpha-\left(\wt\chi+\chi_t^{-1}\right)S_t/\sigma\|^2_{\wt\chi+\chi_t}\right)d\alpha\\
% =&\left(\frac{\det\left(\wt\chi\right)}{\det\left(\wt\chi+\chi_t\right)}\right)^{1/2}\exp\left(\frac{1}{2}\|S_t/\sigma\|^2_{\left(\wt\chi+\chi_t\right)^{-1}}\right)
% \end{align*}
% Since $\E\left[M_\tau\right]\leq 1$ we have
% \begin{align*}
% \Prob\left(\|S_\tau\|^2_{\left(\wt\chi+\chi_\tau\right)^{-1}}\leq 2\sigma\log\left(\frac{\det\left(\wt\chi+\chi_\tau\right)^{1/2}}{\delta\det\left(\wt\chi\right)^{1/2}}\right)\right)
% \leq \frac{\E\left[\exp\left(\frac{1}{2}\|S_\tau/\sigma\|^2_{\left(\wt\chi+\chi_\tau\right)^{-1}}\right)\right]}{\left(\frac{\det\left(\wt\chi+\chi_\tau\right)}{\delta\det\left(\wt\chi\right)}\right)^{1/2}}\leq \delta
% \end{align*}
% Where the Markov inequality is deployed for the final step. 
% The stopping is considered to be the time step as the first time in the sequence when the concentration in the Lemma.~\ref{lem:self} does not hold. 
% \end{proof}





% %%%%%%%%
% \begin{proof}[Proof of Lemma \ref{lem:conf}]
% Given the estimator $\wh\omega_t$ we have the following:
% \begin{align*}
% \wh\omega_t&=\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\left(\mathbf{\Phi}_i\omega^* + \wb\nu_i\right)\right)\\
% &=\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\wb\nu_i\right)\\
% &+ \left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)\omega^*\\
% &-\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\omega^*\\
% \end{align*}
% therefore, for any vector $\zeta\in\Re^d$
% \begin{align*}
% \zeta^\top\wh\omega_t-\zeta^\top\omega^*&=\zeta^\top\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\sum_i^t\left(\mathbf{\Phi}_i^\top\wb\nu_i\right)\\
% &-\zeta^\top\lambda\left(\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i+\lambda I\right)^{-1}\omega^*
% \end{align*}
% As a results, 
% applying Cauchy-Schwarz inequality and inequalities $\|\omega^*\|_{\wo\chi_t^{-1}}\leq \frac{1}{\lambda\left(\wo\chi_t\right)}\|\omega^*\|_2\leq \frac{1}{\lambda}\|\omega^*\|_2$ we get
% \begin{align*}
% |\zeta^\top\wh\omega_t-\zeta^\top\omega^*|&\leq\|\zeta\|_{\wo\chi_t^{-1}}\|\sum_i^t\left(\mathbf{\Phi}_i^\top\wb\nu_i\right)\|_{\wo\chi_t^{-1}}+\lambda\|\zeta\|_{\wo\chi_t^{-1}}\|\omega^*\|_{\wo\chi_t^{-1}}\\
% &\leq \|\zeta\|_{\wo\chi_t^{-1}}\left(\|\sum_i^t\left(\mathbf{\Phi}_i^\top\wb\nu_i\right)\|_{\wo\chi_t^{-1}}+\lambda^{1/2}\|\omega^*\|_2\right)
% \end{align*}
% where applying self normalized Lemma \ref{lem:self}, with probability at least $1-\delta$
% \begin{align*}
% |\zeta^\top\wh\omega_t-\zeta^\top\omega^*|\leq \|\zeta\|_{\wo\chi_t^{-1}}\left(2\sigma\log\left(\frac{\det\left(\wo\chi_t\right)^{1/2}}{\delta\det\left(\wt\chi\right)^{1/2}}\right)+\lambda^{1/2}L_\omega\right)
% \end{align*}
% hold for any $\zeta$. By plugging in $\zeta=\wo\chi_t\left(\wh\omega_t-\omega^*\right)$ %we get the statement in the Lemma \ref{lem:conf}.
% we get the following;
% \begin{align*}
% \|\wh\omega_t-\omega^*\|_{\wo\chi_t}\leq\theta_t(\delta)= \sigma\sqrt{2\log\left(\frac{\det(\wo\chi_t)^{1/2}\det(\lambda I)^{-1/2}}{\delta}\right)}+\lambda^{1/2}L_\omega
% \end{align*}
% The $\det(\wo\chi_t)$ can be written as $\det(\wo\chi_t)=\prod_j^d\alpha_j$ therefore, $trace(\wo\chi_t)=\sum_j^d\alpha_j$. We also know that;
% \begin{align*}
%     (\prod_j^d\alpha_j)^{1/d}\leq \frac{\sum_j^d\alpha_j}{d}
% \end{align*}
% A matrix extension to Lemma 10 and 11 in \cite{abbasi-yadkori2011improved} results in  $\det(\wo\chi_t)\leq \left(\frac{trace(\wo\chi_t)}{d}\right)^d$ while we have $trace(\wo\chi_t)=trace(\lambda I)+\sum_i^t\mathbf{\Phi}_i^\top\mathbf{\Phi}_i\leq d\lambda+tL$, 
% \begin{align}\label{eq:deter}
%     \det(\wo\chi_t)\leq \left(\frac{d\lambda+tL}{d}\right)^d
% \end{align}


% therefore the main statement of Lemma \ref{lem:conf} goes through.
% \end{proof}



% % \eb{Wait, I'm confused. I thought we just proved Lemma 3. And the below is not stated as a lemma. Could you clarify please?}

% % \begin{lemma}[Determinant inequality]
% % For a matrix problem in Eq.~\ref{eq:Bayesian_model}, given a sequence of $\lbrace\mathbf{\Phi}_i,\mathbf{R}_i\rbrace_{i=1}^{t}$, and under $trace{\mathbf{\Phi}(\cdot)\mathbf{\Phi}(\cdot)^\top}\leq L$  we have:
% % \begin{align*}
% % \det\left(\wo\chi_t\right)\leq (\lambda+tL^2/d)^d\quad,\quad \sum
% % \end{align*}
% % \end{lemma}


% % \textbf{BayesReg}_T:&=\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[\phi(x_t^1,\pi_t(x_t^1))^\top \omega(\pi_t)-\phi(x_t^1,\pi_t(x_t^1))^\top \omega^* \big|\mathcal{H}_t\right]\right]\\
% % &\sum_t^T \E_{\mathcal{H}_t}\left[\E_{\omega^*}\left[\phi(x_t^1,\pi_t(x_t^1))^\top \left(\wt\omega_t(\pi_t)-\omega^*\right) \big|\mathcal{H}_t\right]\right]
% % \end{align*}







% \begin{proof}~Lemma.~\ref{lemma:DeterminantLemma}
% We have the following for the determinant of $\det\left(\wo\chi_T\right)$

% \begin{align*}
% \det\left(\wo\chi_T\right)&=\det\left(\wo\chi_{T-1}+\mathbf{\Phi}_T^\top\mathbf{\Phi}_T\right)\\
% &=\det\left(I_H+\mathbf{\Phi}_T\wo\chi_t^{-1}\mathbf{\Phi}_T^\top\right)\det\left(\wo\chi_{T-1}\right)\\
% &=\prod_t^T\det\left(I_H+\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top\right)\det\left(\wt\chi\right)
% \end{align*}
% From linear algebra, and given a time step $t$, we know the characteristic polynomial of the matrix $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ is $CP_t(\wb\lambda)=\det(\wb\lambda I_H-\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top)$. If the set $\lbrace\lambda_1,\lambda_2,\ldots,\lambda_d\rbrace$ represent the eigenvalues of $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ where $\lambda_i\geq\lambda_j$ if $i\geq j$, one can rewrite $CP_t(\wb\lambda)$ as follows;
% \begin{align*}
%     CP(\wb\lambda) = (\wb\lambda-\lambda_1)(\wb\lambda-\lambda_2)\cdots (\wb\lambda-\lambda_H)
% \end{align*} 
% by adding the matrix $I_H$ to $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ where $\lambda_i\geq\lambda_j$, we get $CP_t'(\wb\lambda)=\det(\wb\lambda I_H-I_H-\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top)$, therefore;
% \begin{align*}
%     CP_t'(\wb\lambda) = (\wb\lambda-1-\lambda_1)(\wb\lambda-1-\lambda_2)\cdots (\wb\lambda-1-\lambda_H)
% \end{align*} 
% and the eigenvalues of $I_H+\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ are shifted eigenvalues of $\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top$ by $+1$, i.e. $\lbrace\lambda_1+1,\lambda_2+1,\ldots,\lambda_d+1\rbrace$. Since $\xi^\top\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top\xi=\left(\mathbf{\Phi}{\wo\chi_t^{-1/2}}^\top\xi\right)^\top\left(\mathbf{\Phi}{\wo\chi_t^{-1/2}}^\top\xi\right)$ all the eigenvalues $\lbrace\lambda_1,\lambda_2,\ldots,\lambda_d\rbrace$ are non-negative. As a results,
% \begin{align*}
%     \det\left(I_H+\mathbf{\Phi}_t\wo\chi_t^{-1}\mathbf{\Phi}_t^\top\right)\geq \left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)
% \end{align*}
% As a consequence; 
% \begin{align*}
%     \det\left(\wo\chi_T\right)\geq\det\left(\wt\chi\right) \prod_t^T\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)
% \end{align*}
% Moreover we have
% % \begin{align}
% % \sum_t^T\log\left(1+\|\phi(X_t^1,\pi_t(X_t^1))^\top\|_{\wo\chi_t^{-1}}\right)\leq \sum_t^T\log\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)
% % \end{align}

% \begin{align}%\label{eq:xx}
% 2\sum_t^T\log\left(1+\|\mathbf{\Phi}_t\|_{\wo\chi_t^{-1}}\right)\leq 2\left(\log\left(\det\left(\wo\chi_T\right)\right)-\log\left(\det\left(\wt\chi\right)\right)\right)\leq 2 d\log(\lambda + TL^2/d)
% \end{align}

% and the statement follows.



% \end{proof}










==> acknowledgement.tex <==
% !TEX root = MasterNips.tex

%\vspace{-0.05in}
\section{Acknowledgement}
K. Azizzadenesheli is supported in part by NSF Career Award CCF-1254106. A. Lazaric is supported in part by a grant from CPER Nord-Pas de Calais/FEDER DATA Advanced data science and technologies 2015-2020, CRIStAL (Centre de Recherche en Informatique et Automatique de Lille), and the French National Research Agency (ANR) under project ExTra-Learn n.ANR-14-CE24-0010-01. A. Anandkumar is supported in part by Microsoft Faculty Fellowship, Google faculty award, Adobe grant, NSF Career Award CCF- 1254106, and AFOSR YIP FA9550-15-1-0221.


==> figures.tex <==
\begin{figure}[t!]
\small
\begin{center}
\begin{psfrags}
\psfrag{x1}[][1]{$x_t$}
\psfrag{x2}[][1]{$x_{t+1}$}
\psfrag{x3}[][1]{$x_{t+2}$}
\psfrag{y1}[][1]{$\vec{y}_t$}
\psfrag{y2}[][1]{$\vec{y}_{t+1}$}
\psfrag{r1}[][1]{$\vec{r}_t$}
\psfrag{r2}[][1]{$\vec{r}_{t+1}$}
\psfrag{a1}[][1]{$a_{t}$}
\psfrag{a2}[][1]{$a_{t+1}$}
\includegraphics[width=0.6\textwidth,natwidth=810,natheight=642,trim={-1cm 0cm 0 11cm},clip]{Fig/MulitagentMDP.eps}
\end{psfrags}
\end{center}
\vspace{-0.2in}
\caption{Graphical model of a Cooperative Multi Agent MDP.}
\label{fig:pds2}
\end{figure}

==> old-3.1-TSvsE.tex <==
\section{Thompson Sampling vs \texorpdfstring{$\varepsilon-$}{}greedy}
In this section, we enumerate a few benefits of \TS over $\varepsilon$-greedy strategies. We show how \TS strategies exploit the uncertainties and expected returns to design a randomized exploration while $\varepsilon-$greedy strategies disregard all these useful information for the exploration.
\begin{figure*}[h]
  \begin{minipage}[]{0.33\textwidth}
	 \centering
\includegraphics[width=1.\linewidth]{Fig/secondbest.png}
(a)
  \end{minipage}\hfill
  \begin{minipage}{0.33\textwidth}
     \centering
	 \includegraphics[width=1.\linewidth]{Fig/lowestpicked.png}
     (b)
  \end{minipage}
  \begin{minipage}{0.33\textwidth}
     \centering
     \vspace{-0.8cm}
\includegraphics[width=0.80\linewidth]{Fig/maze1.eps}
(c)
  \end{minipage}
   \caption{A cartoon on \TS vs $\varepsilon$-greedy. The red crosses are the target values, the diamonds are the mean of estimated Q-values with blue intervals as uncertainties (e.g. $c\cdot variance$). $(a)$ $\varepsilon$-greedy strategy mostly chooses the greedy action, action $1$ and explore actions $5,6$ as much as actions $2,3,4$, while \TS randomizes mostly over actions $1,2,3,4$ barely explore actions $5,6$. $(b)$ \bdqn computes the posterior using recent experiences in the replay buffer. Therefore, lack of samples of action $6$ increases the uncertainty on the estimated value and \bdqn explores it again. This further exploration is crucial since the target value changes over time. $(c)$ maze.
}
\label{fig:uncertainty}
\end{figure*}
In order to make a balance between exploration and exploitation, \TS explores actions with higher estimated return with higher probability. In order to exploit the estimated uncertainties, \TS dedicates a higher chance to explore an action if its uncertainty increases. Fig.~\ref{fig:uncertainty}\textit{(a)} expresses the agent's estimated values and uncertainties for the available actions at a given state $x$. While $\varepsilon-$greedy strategy mostly focuses on the greedy action, action $1$, the \TS based strategy randomizes, mostly, over actions $1$ through $4$, utilizes their approximated expected returns and uncertainties, and with low frequency explores actions $5$, $6$. On the other hand, $\varepsilon-$greedy strategy explores actions $5$ and $6$, the actions that the RL agent is almost sure about their low expected returns, as frequent as other sub-greedy actions $2,3,4$ which increases its samples complexity. Moreover, a $\varepsilon-$greedy strategy requires a deep network to approximate the value of all the sub-greedy actions equally good, therefore, it dedicates the network capacity to accurately estimate the values of all the sub-greedy actions equally good, instead of focusing more on the actions with higher promising estimated value. Therefore, it ends up with not accurate enough estimation of other good actions compared to the greedy action.


In a study of value-based deep RL, e.g. \DQN, the network is following a target value which is updated occasionally. Therefore, \TS based strategy should not estimate the posterior distribution which adaptively follows the target values. A commonly used technique in deep RL is a moving window of replay buffer to store the recent experiences. The \TS based agent, after a few tries of actions $5$ and $6$, builds a belief in the low return of these actions given the current target values, while it is possible that later on, the target value suggests a high expected return of these actions. Since the replay buffer is bounded moving window, lack of samples of these actions pushes the posterior belief of these actions to the prior belief, over time, and the agent tries them again in order to update its belief.

Fig.~\ref{fig:uncertainty}\textit{(b)} shows that the lack of samples for action $6$ in the replay buffer, increases the uncertainty of this action and a randomized \TS strategy starts to explore them over. It means that due to adaptive change of target value, respectively the objective, and limited replay buffer, the \bdqn agent is never too confident about the expected return of poor actions and keeps exploring them once in a while.
%
In general, \TS based strategy advances the exploration-exploitation balance by making a trade-off between the expected returns and the uncertainties, while $\varepsilon-$greedy strategy ignores all of this information.

% \begin{figure*}[t]
% \centering
% \hspace*{-1.5cm}
% \subfigure[]{
% \includegraphics[width=.4\textwidth]{Fig/secondbest.png}
% }
% \hspace*{-1.cm}
% \subfigure[]{
% \includegraphics[width=.4\textwidth]{Fig/lowestpicked.png}
% }
% \hspace*{-1.0cm}
% \subfigure[]{
% \includegraphics[width=.34\textwidth]{Fig/maze1.eps}
% }
% \caption{A cartoon representation of \TS vs $\varepsilon$-greedy. The red crosses are the true Q-values, the diamonds are the mean of estimated Q-values with blue intervals as uncertainties (e.g. $c\cdot variance$)}
%    \label{fig:uncertainty}
% \end{figure*}




Another benefit of \TS over $\varepsilon$-greedy can be described using Fig.~\ref{fig:uncertainty}\textit{(c)}. Consider a deterministic and episodic maze game, with episode length $H$ of the shortest pass from the start to the destination. The agent is placed to the start point at the beginning of each episode where the goal state is to reach the destination and receive a reward of $1$ otherwise the reward is $0$. Consider an agent, which is given a  set of Q-functions where the true Q-function is within the set and is the most optimistic function in the set. The agent is supposed to find a $Q$ from this set which maximizes the average return. It is worth noting that the agent task is to find a good function from a function set. %In this situation, the optimism based strategy, with no exploration, chooses the true Q-function at first place, reaches to the endpoint for all the rounds. 

In this situation, \TS randomizes over the Q-functions with high promising returns and relatively high uncertainty, including the true Q-function. When the \TS agent picks the true Q-function, it increases the posterior probability of this Q-function because it matches the observation. When the \TS agent chooses other functions, they predict deterministically wrong values and the posterior update of those functions set to zero. Therefore, the agent will not choose these functions again, i.e. \TS finds the true Q-function by transferring the information through posterior update which helps the agent to find the optimal Q very fast. For $\varepsilon$-greedy agent, even though it chooses the true function at the beginning (it is the optimistic one), at each time step, it randomizes its action with the probability $\varepsilon$. Therefore, it takes exponentially many trials in order to get to the target in this game.

% \begin{figure}[h]
% \centering
%    \begin {minipage}{0.5\textwidth}
% 	 \includegraphics[width=.6\linewidth]{Fig/maze1.eps}
%      \vspace*{-0.5cm}
%    \end{minipage}
%    \caption{maze}
%    \label{fig:maze}
% \end{figure}








% Another superiority of \TS over $\varepsilon$-greedy can be described using Fig.~\ref{fig:uncertainty}\textit{(c)}. Consider an episodic maze-inspired deterministic game, with episode length of shortest pass from the start point to the destination, where the agent is placed to the start point at the beginning of each round the goal state is exiting form the destination. Let us further consider that the shortest path from starting point to the end point has a length of $H$ and the duration of each round is exactly $H$. If the agent reaches the goal state in the $H$ time step, it wins the game and receives a score of $1$, otherwise, it receives $0$. After each $H$ times step, the agent's location is reset to the starting point. Consider an agent, which is given a set of Q-functions where the true Q-function is within the set and is the most optimistic function in the set. %In this situation, the optimism based strategy, with no exploration, chooses the true Q-function at first place, reaches to the endpoint for all the rounds. 
% In this situation, \TS randomizes over the Q-functions with high promising returns and relatively low uncertainty, including the true Q-function. When it picks the true Q-function, it increases the posterior probability of this Q-function, since it matches the likelihood. When \TS chooses other functions since they predict deterministically wrong values, the posterior update of those functions set to zero posteriors, therefore, the model will not choose them again, i.e. \TS finds the true Q-function very fast. For $\varepsilon$-greedy based agent, even though it chooses the true function right away from the begging (it is the optimistic one), at each time step, it randomizes its action whit probability $\varepsilon$. Therefore, it takes exponentially many trials in order to get to the target in this game.

% % \begin{figure}[h]
% % \centering
% %    \begin {minipage}{0.5\textwidth}
% % 	 \includegraphics[width=.6\linewidth]{Fig/maze1.eps}
% %      \vspace*{-0.5cm}
% %    \end{minipage}
% %    \caption{maze}
% %    \label{fig:maze}
% % \end{figure}







